Building A Trusted Execution Environment for In-Storage Computing

In-storage computing with modern solid-state drives (SSDs) enables developers to offload programs from the host to the SSD. It has been proven to be an effective approach to alleviating the I/O bottleneck. To facilitate in-storage computing, many frameworks have been proposed. However, few of them consider security as the priority for in-storage computing. Specifically, since modern SSD controllers do not have a trusted execution environment, an offloaded (malicious) program could steal, modify, and even destroy the data stored in the SSD. In this paper, we first investigate the attacks that could be conducted by offloaded in-storage programs. To defend against these attacks, we build IceClave, a lightweight trusted execution environment for in-storage computing. IceClave enables security isolation between in-storage programs and flash management functions. IceClave also achieves security isolation between in-storage programs and enforces memory encryption and integrity verification of in-storage DRAM with low overhead. To protect data loaded from flash chips, IceClave develops a lightweight data encryption/decryption mechanism in flash controllers. We develop IceClave with a full system simulator and evaluate IceClave with a variety of data-intensive applications. Compared to state-of-the-art in-storage computing approaches, IceClave introduces only 7.6% performance overhead, while enforcing security isolation in the SSD controller with minimal hardware cost. IceClave still keeps the performance benefit of in-storage computing by delivering up to 2.31$\times$ better performance than the conventional host-based trusted computing approach.

==> IceClave (arxiv extended abstract)/abstract.tex <==
\begin{abstract}
In-storage computing with modern solid-state drives (SSDs)   
enables developers to offload programs from the host to the 
SSD. It has been proven to be an effective approach to alleviating the I/O bottleneck. 
To facilitate in-storage computing, many frameworks have been proposed. 
However, few of them treat the 
in-storage security as the first citizen. 
Specifically, since modern SSD controllers do not have a trusted execution environment, 
an offloaded (malicious) program could steal, modify, and even destroy the data stored in 
the SSD. 

In this paper, we first investigate the attacks that could be conducted by offloaded in-storage 
programs. To defend against these attacks, we build a lightweight trusted
execution environment, named IceClave for in-storage computing. 
IceClave enables security isolation between in-storage programs and flash management functions.  
IceClave also achieves security isolation between in-storage programs and enforces
memory encryption and integrity verification of in-storage DRAM with low overhead. To protect data loaded from flash chips,   
IceClave develops a lightweight data encryption/decryption mechanism in flash controllers.  
We develop IceClave with a full system simulator. 
We evaluate IceClave with a variety of 
data-intensive applications such as databases.
Compared to state-of-the-art in-storage computing approaches, 
IceClave introduces only 7.6\% performance overhead, while enforcing security isolation in 
the SSD controller with minimal hardware cost.  
IceClave still keeps the performance benefit of in-storage computing by delivering up to 2.31$\times$
better performance than the conventional host-based trusted computing approach.

\end{abstract}


==> IceClave (arxiv extended abstract)/ack.tex <==
\begin{acks}
We thank the anonymous reviewers for their comments and feedback. This work was 
partially supported by NSF grant CNS-1850317 and CCF-1919044, a gift fund from SK Hynix, and the Department of Defense under Contract FA8075-14-D-0002-0007, TAT 15-1158.
\end{acks}

==> IceClave (arxiv extended abstract)/alltogether.tex <==
\subsection{Put It All Together}
\label{subsec:all}


We illustrate the entire workflow of running an in-storage program with IceClave in Figure \ref{fig:workflow}. 
%The end users rely on IceClave library to offload their programs to the shared SSD. 
Similar to existing in-storage computing frameworks~\cite{willow, biscuit}, IceClave library 
has a host-to-device communication layer based on PCIe, which allows users to transfer data between 
the host and SSD. As discussed in {$\S$\ref{sec:threatmodel}}, we utilize the secure channel developed in 
modern cloud computing platforms for interactions between the host and shared SSD.
%The \texttt{OffloadCode} API (\circlep{1}) described in $\S$\ref{subsec:runtime} is called 
The \texttt{OffloadCode} API (\circlep{1}) described in $\S$\ref{subsec:runtime} is called to offload programs. 
Its parameter \texttt{bin} represents the pre-compiled program in the form of machine code, and
\texttt{lpa} is a list of Logical Page Addresses (LPAs) of data needed by the offloaded program.
It uses task ID (\texttt{tid}) as an index for identifying the offloaded procedure.

IceClave runtime will create a new TEE for the offloaded program using \texttt{CreateTEE} ({\circlep{2}}). 
At creation, IceClave runtime will allocate memory pages from the normal memory region to the TEE, while 
the TEE metadata will be initialized and maintained in the secure memory region. IceClave also executes  
\texttt{SetIDBits} to set access permissions in the address mapping table for {LPAs}. 
%specifying page table address, program identity and other security info. 
%The user program binary will be copied into the TEE after the TEE is successfully initialized.     
The TEE does not rely on FTL to get physical page addresses (see $\S$\ref{subsec:ftl}),  
as it can access the mapping table in the protected memory region (\circlep{3}). 

However, the in-storage program may occasionally encounter cache misses, when a mapping entry for the accessed 
LPA is not cached in the SSD DRAM. In this case, the TEE has to redirect the address translation request 
to the FTL via \texttt{ReadMappingEntry} (\circlep{4}). This TEE will be paused and switched to the secure world, such 
that FTL will load the missing mapping table pages (\circlep{5}), update the cached mapping table in the protected memory 
region, and return the PPA to the TEE. To avoid in-storage programs probing the entire physical space 
of the SSD, we enforce the access control (see $\S$\ref{subsec:mapping}). 
Any data on the data path to the TEE is encrypted with the stream cipher engine (\circlep{6}). Note that 
users are encouraged to encrypt their data to defend against attacks from malicious host OS. They will send their decryption key to 
the TEE along with the offloaded program, and decrypt the data at runtime in the TEE. 
%Above security enforcement measures are managed automatically by IceClave without user notice.
\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/workflow.pdf}
	\vspace{-2ex}
	\caption{IceClave workflow of running in-storage programs. In this diagram, IceClave Runtime and Library, TEE, FTL, Stream Cipher Engine, and Flash Controller are compute regions. Mapping Table and Flash are memory regions.
	}
	\label{fig:workflow}
		\vspace{-3ex}
\end{figure}
The TEE will be invoked by IceClave runtime once the in-storage program is readily prepared inside the TEE. 
IceClave runtime constantly monitors the status of initiated TEEs, secures memory regions, and ensures the 
mapping table permission guard. Exceptions will be thrown out if any aforementioned integrity is compromised. 

During the entire lifecycle of a TEE, the hardware protection mechanisms described in $\S$\ref{subsec:memory} 
are enforced to prevent physical memory attacks. IceClave will also enforce strong isolation between 
TEEs and the FTL. The memory protection described in $\S$\ref{subsec:ftl} will also be enforced in existing 
TrustZone memory controller (TZASC)~\cite{TZASC}. Once reaching the end of the TEE program, 
the results are copied into the TEE's metadata region before terminating the TEE and reclaiming used resources (\circlep{8}). 
IceClave will initiate a DMA transfer request to the host using NVMe interrupts, signaling the readiness of results. 
Results are returned to the host memory via \texttt{GetResult} (\circlep{7}) provided in IceClave library.



==> IceClave (arxiv extended abstract)/authors.tex <==
%%%%%% group affiliations %%%%%%%
\author{Yuqi Xue, Luyi Kang\footnotemark[2], Weiwei Jia, Xiaohao Wang, Jongryool Kim\footnotemark[3], Changhwan Youn\footnotemark[3], \\ Myeong Joon Kang\footnotemark[3], Hyung Jin Lim\footnotemark[3], Bruce Jacob\footnotemark[2], Jian Huang}

\affiliation{%
  \institution{UIUC, \footnotemark[2]University of Maryland, College Park, \footnotemark[3]SK Hynix}
  \streetaddress{Address}
  \city{}
  \state{}
  \country{}}
%\email{luyikang@umd.edu, blj@ece.umd.edu}

% \affiliation{%
%   \institution{\textsuperscript{2}University of Illinois at Urbana-Champaign}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
%\email{{yuqixue2, weiweij, jianh}@illinois.edu, xiaohaow3105@gmail.com}

% \affiliation{%
%   \institution{\textsuperscript{3}SK Hynix}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
%\email{{jongryool.kim, changhwan.youn, myeongjoon.kang, jin.lim}@us.skhynix.com}

% \renewcommand{\shortauthors}{Kang, et al.}
%%%%%% end %%%%%%%%

%%%%%% separate entry for each author
% \author{Luyi Kang}
% \authornote{Co-primary authors.}
% \authornote{Work done while visiting the Systems Platform Research Group at UIUC.}
% \affiliation{%
%   \institution{University of Maryland, College Park}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
% %\email{luyikang@umd.edu}

% \author{Yuqi Xue}
% \authornotemark[1]
% \affiliation{%
%   \institution{UIUC}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
% %\email{yuqixue2@illinois.edu}

% \author{Weiwei Jia}
% \authornotemark[1]
% \affiliation{%
%   \institution{UIUC}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
% %\email{weiweij@illinois.edu}

% % [TODO]
% \author{Xiaohao Wang}
% \authornote{Now at NVIDIA.}
% \affiliation{%
%   \institution{UIUC}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
% %\email{xiaohaow3105@gmail.com}

% \author{Jongryool Kim}
% \affiliation{%
%   \institution{SK Hynix}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
% %\email{jongryool.kim@us.skhynix.com}

% \author{Changhwan Youn}
% \affiliation{%
%   \institution{SK Hynix}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
% %\email{changhwan.youn@us.skhynix.com}

% \author{Myeong Joon Kang}
% \affiliation{%
%   \institution{SK Hynix}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
% %\email{myeongjoon.kang@us.skhynix.com}

% \author{Hyung Jin Lim}
% \affiliation{%
%   \institution{SK Hynix}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
% %\email{jin.lim@us.skhynix.com}

% \author{Bruce Jacob}
% \affiliation{%
%   \institution{University of Maryland, College Park}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
% %\email{blj@ece.umd.edu}

% \author{Jian Huang}
% \affiliation{%
%   \institution{UIUC}
%   \streetaddress{Address}
%   \city{}
%   \state{}
%   \country{}}
% %\email{jianh@illinois.edu}

\renewcommand{\shortauthors}{} % L. Kang, Y. Xue, W. Jia, X. Wang, J. Kim, C. Youn, M. Kang, H. Lim, B. Jacob, J. Huang}

==> IceClave (arxiv extended abstract)/background.tex <==
\section{Background and Motivation}
\label{sec:motivation}
In this section, we first introduce the background of flash-based SSDs and 
in-storage computing, and discuss why it is desirable to have TEEs 
for in-storage computing. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{./figures/ssdhardware.pdf}
    \vspace{-2ex}
    \caption{Internal architecture of flash-based SSDs.}
    \label{fig:ssd-arch}
    \vspace{-3ex}
\end{figure}


\subsection{Flash-Based Solid-State Drive}
\label{subsec:ssd}

%Flash-based SSDs provide significant performance improvement %up to 5,000$\times$ higher throughput and up to 100$\times$ lower latency
%than conventional hard-disk drives (HDDs), while their price is fast approaching to that of HDDs.
The rapidly shrinking process technology has allowed SSDs to boost their performance
and capacity, which accelerates their adoption in commodity systems such as data 
centers today~\cite{flashblox, flashmap:isca2015, flatflash:asplos2019}.
We present a typical SSD architecture in Figure~\ref{fig:ssd-arch}.
An SSD has three major components: a set of flash memory packages,
an SSD controller having embedded processors with DRAM, and flash controllers~\cite{chen2011essential, 
deepstore:micro2019}. The flash packages are
organized in a hierarchical manner. Each SSD has multiple channels. 
%where each channel can receive and process read/write commands independently. 
Each channel is shared by multiple flash
packages. Each package consists of multiple flash chips. Each chip has multiple planes. Each plane
is divided into multiple flash blocks, each of which consists of multiple flash pages.


Due to the nature of flash memory,
when a free flash page is written once, that page is no longer available for future writes until
that page is erased.
However, erase operation can be performed only at a block %(which has 64 or more pages) 
granularity, which is time-consuming.
Thus, writes are issued to free pages that have been erased (i.e., out-of-place write) rather than
waiting for the expensive erase operation. 
Garbage collection (GC) will be performed later to clean the obsolete data in SSDs.
As each flash block has limited endurance,
it is important for blocks to age uniformly (i.e., wear leveling).
SSDs employ out-of-place write, GC, and wear leveling to overcome the shortcomings
of SSDs and maintain indirections for indexing the logical-to-physical address mapping.
All these are managed by the Flash Translation Layer (FTL) in the SSD controller.



\subsection{In-Storage Computing}
\label{subsec:instorage}
We have long recognized the inefficiency of traditional CPU-centric computing 
for data-intensive applications that need to transfer large amounts of 
data from storage.
The application performance is limited by the low bandwidth of 
PCIe interface between the host and SSD. % such as PCIe.
To tackle this challenge, various in-storage computing 
approaches~\cite{biscuit, summarizer, willow, capi:2014:whitepaper, deepstore:micro2019} have been proposed.
With them, we can process data by exploiting SSD processors and high internal 
bandwidth of flash chips. %without going through the slow I/O interface. 
Their significant performance benefits show that in-storage 
computing is a promising technique. 

However, as in-storage processors operate independently from the host,  
it poses security challenges to the adoption of in-storage computing, especially in 
the multi-tenancy setting where multiple application instances share the physical 
SSD~\cite{multissd:sigmod2014, documentdb:vldb2015, cloudstorage:osdi2012, libra:eurosys2014, 
slo:fast2015, heracles:isca2015}. 



%\subsection{In-Storage Vulnerabilities and Why In-\\Storage TEE}
\subsection{In-Storage Vulnerabilities}
\label{subsec:why}
%As discussed in existing in-storage computing frameworks~\cite{biscuit, willow}, 
When specific code is offloaded to in-storage processors, a copy of the privilege information is transferred and maintained in the DRAM of the SSD controller~\cite{biscuit,willow}. 
Such a solution is developed under the assumption that the offloaded code has already 
known the address and size of the accessed data in advance.
However, %a malicious program can still intentionally access other data regions inside the SSD 
adversaries can exploit in-storage software and firmware vulnerabilities such as 
buffer overflows~\cite{sok, pointerguard:security2003, bufferoverflow},  
and bus-snooping attack~\cite{ssdflaw} to achieve privilege escalation. After that, 
they can conduct various further attacks.  
We present them in the following. 

\begin{itemize}[leftmargin=*]
    \item {A malicious user can manipulate the intermediate data and output generated 
    	by in-storage programs via both software and physical attacks, causing incorrect computing results. }
\vspace{1ex}
	\item {A malicious program can 
		%manipulate the critical data structures (e.g., mapping 
		%table in FTL) stored in the shared SSD DRAM, and 
		intercept FTL functions like GC and 
	        wear leveling in the SSD and mangle the flash management. This would cause data loss 
		or device destroyed. } 
\vspace{1ex}
	\item {A malicious user can steal user data stored in flash chips via physical attacks 
	like bus snooping attack, when 
		in-storage programs load data from flash chips to SSD DRAM. }
		%even destroy the entire SSD by manipulating the core functions in the FTL. }
		\vspace{1ex}
		
\end{itemize}

To defend against these attacks, an alternative solution is to develop an OS or hypervisor for 
in-storage computing. However, due to the limited resources  
in the SSD controller, running a full-fledged OS can introduce significant overheads to the SSD and increase the attack surface, due to its large codebase.
%it is not easy to run an full-fledged OS, while supporting the execution of 
%in-storage programs efficiently. 
Moreover, these techniques are not sufficient to defend against the aforementioned attacks such as 
board-level physical attacks.
As we move compute closer to storage devices, it is highly desirable to have a lightweight execution environment 
for this non-traditional computing paradigm.


Since SSDs were designed with the assumption they are hardware 
isolated from the host and purely used as storage rather than computing, 
modern computing systems do not provide secure runtime environment for in-storage computing.
As discussed in $\S$\ref{sec:intro}, a straightforward approach is to adopt the SGX-like solutions~\cite{www:intelsgx,keystone:eurosys2020}. 
However, this requires significant hardware changes and even replacement of storage processors available in modern SSDs. 
As SGX was developed as a generic framework for host machines, it is hard to achieve optimal performance for 
in-storage programs. 

%ARM processors 
%available in modern SSD controllers provide the TrustZone technique~\cite{trustzone} to enable 
%the creation of secure world 
%and normal world, however, it is unclear whether and how it can be utilized for in-storage computing, and 
%how it should work seamlessly together with the hardware components in SSD controllers.  
%And most importantly, TrustZone cannot defend against physical attacks. 
%Therefore, 
%%as we move computation to the SSD controller, 
%we have to rethink their system design with considering the security as the first citizen. 
%%and develop TEEs for in-storage programs.  




==> IceClave (arxiv extended abstract)/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
%This paper investigates security vulnerabilities for in-storage computing. 
Due to the lack of TEE support in SSD controllers, 
adversaries can intervene offloaded programs, mangle flash management, steal and destroy user data.
%As we move forward to in-storage computing for practical 
%benefits, we have to address these security challenges.
To this end, %we develop a
we develop IceClave, a
lightweight TEE which enables security
isolation between in-storage programs and flash management.
IceClave can also defend 
against physical attacks with minimal hardware cost.
%With running data-intensive 
%applications, we show IceClave introduces minimal overhead to application performance,  
%while ensuring security guarantees for in-storage computing.
%\hl{Our evaluation shows} IceClave \hl{ensures security guarantees for in-storage computing programs while incurring minimal overhead.}



==> IceClave (arxiv extended abstract)/design.tex <==
%\vspace{-2ex}
\section{\mbox{\hspace{-0.89ex} Securing In-Storage Computing with IceClave}}
\label{sec:design}
IceClave is a TEE for in-storage computing with minimal performance and hardware cost. It aims to defend against three attacks: (1) the attack against co-located in-storage 
programs; (2) the attack against the FTL; (3) the potential physical attack 
against the data loaded from flash chips and generated by in-storage programs.

\paragraph{Protecting Flash Translation Layer.}
\label{subsec:ftl}
As the FTL manages flash blocks and controls how user data is mapped to each flash page, its protection is crucial. 
If any malicious in-storage programs gain control over it, they can read, erase, or overwrite data from other users, 
causing severe consequences such as data loss and leakage. 

To protect FTL from malicious in-storage programs, we have to guarantee offloaded applications 
cannot access memory regions used by FTL. We can use ARM TrustZone to create secure and normal worlds, and then place FTL functions in the secure world, and place all in-storage applications in the normal world. 
However, this will cause significant performance overhead for in-storage applications. 
This is because when an application accesses a flash page each time, it needs to context switch to the 
secure world which hosts the FTL and its address mapping table. 

To address this challenge,
we partition the entire physical main memory space into 
three memory regions: normal, protected, and secure by extending TrustZone.
We allow FTL to execute in the secure world, and place in-storage applications in the normal world; therefore, they cannot 
access any code or data regions that belong to the FTL. 
We use the protected memory region in the normal world to host the shared address mapping table, such that in-storage applications can only read the mapping
table entries for address translation, without paying the context-switch overhead.
\begin{figure}
	\centering
	\includegraphics[width=0.85\linewidth]{figures/overview.pdf}
	\vspace{-2ex}
	\caption{Overview of IceClave architecture.}
	\label{fig:overview}
%	\vspace{-3ex}
\end{figure}
\paragraph{Enforcing Access Control for In-Storage Programs.}
\label{subsec:mapping}
Although each in-storage program only has the read access permission when accessing the mapping table of 
the FTL, a malicious in-storage program 
could probe the mapping table entries (e.g., by brute-force)
and easily access the data belonging to other in-storage programs.

To address this challenge, we extend the address mapping table of FTL.  
We use the ID bits in each entry (8 bytes per entry) to track the identification of each in-storage TEE, 
and use them to verify whether an in-storage TEE has the permission to access the mapping table entry or not. 
Each in-storage program only has accesses to the address mapping table of the FTL and allocated memory space. 
Accesses to other memory locations will result in a fault in the memory management unit.

\paragraph{Securing In-Storage DRAM.}
\label{subsec:memory}
In-storage programs load data from flash chips to the SSD DRAM for data processing. 
The user data that includes raw data, intermediate data, and produced results in the DRAM could be leaked or tampered with at runtime due to physical attacks. To address this challenge, IceClave enables both memory encryption and integrity verification. 

For memory encryption, the state-of-the-art work usually uses split-counter encryption~\cite{bmt:micro07}, which has significant performance overhead. However, this is less of a concern for in-storage computing because in-storage workloads are mostly read intensive. Based on this observation, we design the hybrid-counter scheme.

The key idea of hybrid-counter is that we only use major counters for read-only pages. For writable pages, we apply the traditional split-counter scheme.
As minor counters will not change as long as the pages are read-only, we do not need minor counters for read-only pages.
In this case, we can improve the counter fetching performance by packing more counters per cache line.

To ensure the processor receives exactly the same content as it wrote in 
the memory most recently, we also enable memory integrity verification by employing Bonsai Merkle Tree (BMT)~\cite{bmt:micro07}. Due to the hybrid-counter scheme, IceClave maintains two Merkle trees, but the extra memory cost is negligible.




\paragraph{IceClave Implementation.}
We show the overview of IceClave architecture in Figure~\ref{fig:overview}.
We extend ARM TrustZone to create secure and normal world for security isolation
and protection of different entities in FTL, while enabling memory
encryption and verification with memory encryption engine (MEE).
We implement IceClave with a computational SSD simulator developed based on the
SimpleSSD, Gem5, and USIMM simulator.
To verify the core functions of IceClave,
we also implement IceClave with an OpenSSD Cosmos+ FPGA board.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/iscvsvanila.pdf}
    \vspace{-3ex}
    \caption{Performance comparison of Host, Host+SGX, ISC, and IceClave (from left to right).}
    \label{fig:iscvsvanila}
    \vspace{-3.5ex}
\end{figure}

\paragraph{Performance of IceClave.}
We evaluate IceClave with a set of synthetic and real-world workloads that are typical for in-storage computing.
We compare IceClave with the following state-of-the-art solutions: (1) host-based computing without security (\texttt{Host}), (2) host with Intel SGX (\texttt{Host+SGX}), and (3) in-storage computing without security (\texttt{ISC}).
As shown in Figure~\ref{fig:iscvsvanila}, IceClave outperforms 
Host and Host+SGX by more than 2.3$\times$, respectively.
Compared to the ISC baseline, IceClave introduces 
7.6\% performance overhead, due to the security techniques used in the in-storage TEE.

==> IceClave (arxiv extended abstract)/evaluation.tex <==
\section{Evaluation}
\label{sec:eval}
Our evaluation demonstrates that: (1) IceClave introduces minimal performance overhead to in-storage workloads while
enforcing security isolation in SSD controllers ($\S$\ref{subsec:perf} and $\S$\ref{subsec:overhead}); 
%(2) It has minimal negative impact on the energy efficiency of
%in-storage computing ($\S$\ref{subsec:power}); 
(2) IceClave scales in-storage application performance as we increase the internal bandwidth
of SSDs ($\S$\ref{subsec:bandwidth}); 
(3) It can benefit various SSD devices with different access latencies ($\S$\ref{subsec:latency});
(4) IceClave still outperforms conventional host-based computing significantly while offering security isolation, 
as we vary the in-storage computing capability ($\S$\ref{subsec:computing} and $\S$\ref{subsec:dram}); 
(5) IceClave enables concurrent execution of multiple in-storage  
programs with low performance overhead ($\S$\ref{subsec:multitenant}). 

\begin{table}
    \centering
    \caption{In-storage workloads used in our evaluation.}
    \vspace{-2ex}
    \scriptsize
    \label{tab:workload}
    \begin{tabular}{|p{45pt}|p{145pt}|}
    \hline
                \textbf{Workload}   & \textbf{Description} \\ \hline
        Arithmetic & Mathematical operations against data records                                  \\ \hline
        Aggregation& Aggregate a set of values with average operation     \\ \hline
        Filter     & Filter a set of data that matches a certain feature                                        \\ \hline
        %Inner Join & Select rows that have matching values in both tables                                      \\ \hline
        TPC-H Q1   & Query pricing summary involving scan                    \\ \hline
        TPC-H Q3   & Query shipping priority involving join              \\ \hline
        TPC-H Q12  & Query shipping modes and order priority with join                                           \\ \hline
        TPC-H Q14  & Query market response to promotion with join                                                 \\ \hline
        TPC-H Q19  & Query discounted revenue with join and aggregate           \\ \hline
        TPC-B      & Queries in a large bank with multiple branches                                  \\ \hline
        TPC-C      & Online transaction queries in a warehouse center                              \\ \hline
        Wordcount  & Count the number of words in a long text~\cite{biscuit} \\ \hline
    \end{tabular}
    	\vspace{-3ex}
\end{table}


\subsection{Experimental Setup}
\label{subsec:setup}
We evaluate IceClave with a set of synthetic workloads and real-world applications as shown in Table~\ref{tab:workload}.
In the synthetic workloads, we use several essential operators in database system, including arithmetic, aggregation, and filter operations.
As for the real-world applications, we run real queries from the TPC-H benchmark. Specifically, we use TPC-H Query 1,
3, 12, 14, and 19 that include the combination of multiple join and aggregate operations.
In addition to these workloads, we also run write-intensive workloads TPC-B, TPC-C, and Wordcount to 
further evaluate the encryption and integrity verification overhead of IceClave.
%\hl{It is worth noting that SSjoin and Decompress are also computation-intensive workloads, which are not 
%great workload candidates for in-storage computing according to our experiments and previous study}~\cite{summarizer}. \hl{Therefore, we exclude these two workloads when we report the average performance results through the paper.}
In all these workloads, we populate their dataset (tables) to
the size of 32GB, and place them across the channels in the SSD. %We collect traces from the workloads running on the baseline system to evaluate their access patterns.


We compare IceClave with several state-of-the-art solutions. Particularly, we compare IceClave with the Intel SGX available in the host machine, in which we
load the data from the SSD to the host memory and conduct the queries in the SGX. For this setting, we use a real server, which has an Intel {i7-7700K}
processor running at 4.2GHz, 16GB DDR4-3600 DRAM, and 1TB Intel DC P4500 SSD. {For fair comparison, we follow the specification of the Intel DC P4500 SSD
to configure our SSD simulator. We also compare IceClave with current in-storage computing approaches that do not provide TEEs for offloaded programs. }
We list them as follows:

\begin{itemize}[leftmargin=*]
\vspace{1ex}
    \item \textbf{Host}: in which we load data from the SSD to the host memory, and execute the data queries using host processors.
        The host machine and SSD setups are described above.
\vspace{1ex}
    \item \textbf{Host+SGX}: in which we run data queries within the Intel SGX after loading data from the SSD. The version of the
            SGX SDK we use in our experiments is 2.5.101.
\vspace{1ex}
    \item \textbf{In-Storage Computing (ISC):} in which we run data queries with the ARM processors
            in the SSD controller, such that we can exploit the high internal bandwidth of the SSD.
\vspace{1ex}
\end{itemize}

%We use CACTI 6.5~\cite{cacti} to
%estimate energy utilization of the SRAM (including the one used for stream cipher engine) in the 32nm technology node.
%We use the \texttt{itrs-hp} model for SRAMs of the SSD.
%We assume the DRAM energy is 20-pJ/bit~\cite{markhorwitz}. We use the power consumption of flash page
%access in the Intel DC P4500 SSD to calculate the energy consumed by flash accesses.
%We obtain the energy consumption of processor and network-on-chip using McPAT~\cite{mcpat}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/iscvsvanila.pdf}
    \vspace{-3ex}
    \caption{Performance comparison of Host, Host+SGX, ISC, and IceClave (from left to right).
    We show the performance breakdown of each scheme.}
    \label{fig:iscvsvanila}
    	\vspace{-3ex}
\end{figure}




\subsection{Performance of IceClave}
\label{subsec:perf}
We show the normalized performance of running each query benchmark in Figure~\ref{fig:iscvsvanila}.
We use the Host as the baseline, in which we run the query workload with the host machine while 
loading the dataset from the SSD. As shown in Figure~\ref{fig:iscvsvanila}, IceClave outperforms 
Host and Host+SGX by 2.31$\times$ and 2.38$\times$ on average, respectively. This shows that 
IceClave will not compromise the performance benefits of in-storage computing. 
%while ensuring the security isolation inside SSDs. 
As those data query workloads are bottlenecked by the storage 
I/O, the SGX on the host machine (Host+SGX) slightly decreases the workload performance. 
Compared to in-storage computing without security isolation enabled (ISC), IceClave introduces 
7.6\% performance overhead, due to the security techniques used in the in-storage TEE. 
%\hl{For these compute-intensive workloads such as SSJoin and decompress, as we expected, they do 
%not obtain performance benefits from in-storage computing. However, we still show that} IceClave \hl{introduces 
%minimal performance overhead in comparison with ISC.}


To further understand the performance behaviors of IceClave, we also demonstrate the performance 
breakdown in Figure~\ref{fig:iscvsvanila}. As for the Host and Host+SGX schemes, we partition their 
workflow into two major parts: data load and computing time. As we can see, 
Host+SGX incurs 103\% extra computing time on average, caused by the SGX running in the host machine. 
As for the ISC and IceClave schemes, we profile the data load time from flash chips, the computing 
time with in-storage processors, and the overhead caused by the memory encryption and verification 
for IceClave. As shown in Figure~\ref{fig:iscvsvanila}, IceClave and ISC take much less time on loading 
time, as the internal bandwidth of the SSD is higher than its external bandwidth. And they require  
more time (2.47$\times$ on average) to execute the data queries. Compared to ISC, IceClave needs memory 
encryption and verification. 
For write-intensive workloads such as Wordcount, IceClave slightly increases memory encryption overhead. This is because Merkle tree intrinsically supports parallel updates, and our hybrid-counter design preserves this property by default.
However, IceClave still 
outperforms host-based approaches significantly for a majority of in-storage workloads. 
%\hl{For the workloads SSJoin and decompress, they 
%incur more memory writes during their computation procedure, the memory encryption and integrity verification 
%cause more overheads. However, this is less of a concern, as }

\begin{table}[t]
    \centering
	\caption{Overhead source of IceClave.}
	\vspace{-2ex}
    \footnotesize
    \label{tab:overhead}
	\begin{tabular}{|p{78pt}<{\raggedleft}|p{55pt}<{\raggedright}|}
        \hline
    	\textbf{Overhead Source}   & \textbf{Average Time} \\ \hline
        TEE creation &  95~$\mu$s                                 \\ \hline
        TEE deletion &   58~$\mu$s   \\ \hline
        Context switch    &  3.8~$\mu$s           \\ \hline
        Memory encryption   &    102.6~ns              \\ \hline
        Memory verification   &  151.2~ns             \\ \hline
    \end{tabular}
    	\vspace{-3ex}
\end{table}

\begin{table}[t]
	\centering
	\footnotesize
	\caption{Extra memory traffic caused by memory encryption and verification when running in-storage workloads.}
	\vspace{-2ex}
	\label{tab:memtraffic}
	\begin{tabular}{|c|c|c|}
		%\toprule
		\hline
		\textbf{Workload} & \textbf{Encryption} & \textbf{Integrity Verification}\\ 
		\hline
 		Arithmetic & 3.05\% & 2.27\% \\
 		\hline
		Aggregate & 3.06\% & 2.26\% \\
		\hline
		Filter & 3.04\% & 2.26\% \\
		\hline
		TPC-H Query 1 & 2.99\% & 2.22\% \\
		\hline
		TPC-H Query 3 & 5.62\% & 4.5\%\\
		\hline
		TPC-H Query 12 & 5.11\% & 3.78\% \\
		\hline
		TPC-H Query 14 & 10.28\% & 5.39\%\\
		\hline
		TPC-H Query 19 & 36.20\% & 24.75\%\\
		\hline
		TPC-B & 46.92\% & 36.68\%\\
		\hline
		TPC-C & 39.09\% & 31.72\%\\
		\hline
		Wordcount & 67.45\% & 43.81\%\\
		\hline
% 		\hline
% 		Arithmetic & 10.3\% & 17.3\% \\
% 		\hline
% 		Aggregate & 9.5\% & 16.6\% \\
% 		\hline
% 		Filter & 9.3\% & 16.4\% \\
% 		\hline
% 		TPC-H Query 1 & 9.9\% & 15.4\% \\
% 		\hline
% 		TPC-H Query 3 & 22.4\% & 34.4\%\\
% 		\hline
% 		TPC-H Query 12 & 20.9\% & 28.5\% \\
% 		\hline
% 		TPC-H Query 14 & 46.7\% & 64.5\%\\
% 		\hline
% 		TPC-H Query 19 & 69.7\% & 81.0\%\\
% 		\hline
% 		TPC-B & 39.6\% & 53.4\%\\
% 		\hline
% 		TPC-C & 37.4\% & 49.6\%\\
% 		\hline
	\end{tabular}
		\vspace{-5ex}
\end{table}



\subsection{Overhead Source in IceClave}
\label{subsec:overhead}
We also profile the entire workflow of running an in-storage program with IceClave.  
We show the critical components of IceClave and their overhead in Table~\ref{tab:overhead}. 
IceClave takes 95~$\mu$s and 58$~\mu$s (measured in real SSD FPGA board) to create and 
delete a TEE inside SSD, respectively. The overhead of context switch between 
secure world and normal world is 3.8~$\mu$s. As discussed in $\S$\ref{subsec:ftl}, 
IceClave has infrequent context switches at runtime, as it places the frequently accessed 
address mapping table in the protected memory region. The context switch happens mostly because 
the mapping table entries are missing in the protected memory region, and IceClave needs to switch 
to the secure world to fetch the mapping table from flash chips, and update 
them in the protected memory region. 

Moreover, IceClave incurs much less memory encryption and verification operations, 
because most in-storage workloads are read intensive (see $\S$\ref{subsec:memory} and Table~\ref{tab:memfootprint}). 
The average execution times of each memory encryption and verification take 102.6~ns and 151.2~ns, respectively.  
%To understand the memory overhead of IceClave, 
We profile the additional memory accesses (see Table~\ref{tab:memtraffic}) 
incurred by fetching and overflowing counters in the memory encryption and integrity verification. 
%Table~\ref{tab:memtraffic} shows 
%the increase of memory traffic caused by memory encryption and integrity verification in percentage, compared to 
%the data traffic. 
We show the extra memory traffic in percentage in Table~\ref{tab:memtraffic}, when comparing to the regular memory traffic without 
enforcing memory security. 
Memory encryption and verification increase the memory traffic by 20.26\% and 14.51\% on average, respectively. 

We also profile the number of flash address translations requested from a TEE, and find that only 0.17\% of these address 
translations are missed in the cached mapping table in the protected memory region. This indicates that in-storage programs do not incur the context 
switch from the normal world to the secure world frequently, showing that IceClave is lightweight for in-storage 
workloads.  


%\subsection{Impact on Power Consumption}
%\label{subsec:power}
%We now evaluate the energy efficiency of IceClave against ISC. 
%%We measure the power consumption of the host processors using an open-source tool CPU %Energy Meter~\cite{powermeter} and \textit{perf}~\cite{rapl}.
%With the measurement methods described in $\S$\ref{subsec:setup}, 
%we collect the energy consumption of the entire SSD, including the energy consumed by embedded processors, SSD DRAM, and 
%flash chips. We present the results in Figure~\ref{fig:energy}. 
%Compared to ISC without security isolation,    
%IceClave introduces up to 11.8\% energy overhead. %as we run various query workloads. 
%
%To further understand the energy consumption of IceClave, we show the energy breakdown of all these schemes in 
%Figure~\ref{fig:energy}. It includes the energy consumption of ARM processor, SSD DRAM, and flash access. %and stream cipher engine. 
%Compared to ISC, the energy overhead of IceClave is mainly caused by the extra operations generated by 
%the memory encryption and verification. The stream cipher engine of IceClave adds trivial energy overhead (0.01\% of the energy consumption of flash access). 

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{figures/energy.pdf}
%	\vspace{-5.5ex} 
%	\caption{Energy overhead of IceClave, normalized to ISC (left).}
%	\label{fig:energy}
%\end{figure}




\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/bws.pdf}
	\vspace{-5ex} 
	\caption{IceClave scales its performance, as we vary the internal SSD bandwidth by using different number of channels (normalized to Host).}
	\label{fig:bws}
		\vspace{-4ex}
\end{figure}



\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/bws-isc.pdf}
	\vspace{-6ex} 
	\caption{IceClave introduces minimal performance overhead (normalized to ISC), as we vary the internal SSD bandwidth by using different number of channels.}
	\label{fig:bws-isc}
		\vspace{-3ex}
\end{figure}

\subsection{Impact of SSD Bandwidth}
\label{subsec:bandwidth}
We now evaluate the performance sensitivity of IceClave, as we change different SSD parameters. 
We first vary the internal bandwidth of the SSD by changing the number of flash channels from 4 to 32. With this, 
the aggregated internal I/O bandwidth grows linearly, while the external bandwidth is 
capped by the PCIe bandwidth~\cite{summarizer, lightnvm}. We compare IceClave with the host-based approach (Host), 
and present the normalized speedup in Figure~\ref{fig:bws}. %As we can see, 
For each data query workload, 
the performance benefit of IceClave scales significantly, as we increase the number of channels. To be specific, 
IceClave speeds up the performance by 1.7--5.0$\times$ over Host, showing that IceClave has negligible 
negative impact on the performance of in-storage computing. As for in-storage workloads that involve 
more complicated computations such as TPC-B, TPC-C, and Wordcount, increasing the internal bandwidth brings 1.2--1.8$\times$ 
performance speedup, and for others such as the synthetic workloads and TPC-H, IceClave obtain more performance benefits (1.9-6.2$\times$).    
Note that IceClave achieves even more performance benefits than Host+SGX, because SGX introduces 
extra overhead (see Figure~\ref{fig:iscvsvanila} and $\S$\ref{subsec:perf}). 
And IceClave enables TEE for in-storage programs.
%\hl{For compute-intensive workloads SSJoin and decompress, we obtain trivial performance improvement as we 
%increase the SSD bandwidth, this is because these workloads are constrained by compute resources rather than I/O bandwidth.}

{As we vary the internal SSD bandwidth, we also compare IceClave with ISC. As shown in Figure}~\ref{fig:bws-isc}, 
{IceClave decreases the application performance by up to 28\% (8.6\% on average), compared to ISC. Its 
additional overhead is slightly 
increased as we increase the number of channels for complicated data queries like TPC-C. This is mainly due to the 
increased overhead of memory encryption and integrity verification. However, IceClave offers a TEE 
for offloaded programs, making us believe it is worth the effort. }



\subsection{Impact of Data Access Latency}
\label{subsec:latency}
To understand how the data access latency affects the performance of IceClave, 
{we vary the read latency of accessing a flash page from 10~$\mu$s, modeling an ultra-low 
latency NVMe SSD}~\cite{memblaze, optane_latency}, to 110~$\mu$s, modeling a commodity TLC-based SSD~\cite{microntlc}. 
We keep the write latency as 300~$\mu$s, this is because most in-storage workloads are read-intensive, 
which involve few write operations to the dataset stored 
in the SSD. We use 8 channels in the SSD. We present the experimental results in Figure~\ref{fig:lat}. 
{As shown in Figure}~\ref{fig:lat}, compared to the host-based computing approach that is bottlenecked by the 
external PCIe bandwidth, IceClave delivers performance benefit (1.8--3.2$\times$) for various 
SSD devices with different access latencies. For TPC-B, TPC-C, and TPC-H Q19 query workloads that 
require more computing resource for hash join operations, IceClave offers less performance 
benefit for the SSD with ultra-low latency, because the processors in the host machine provide more powerful computing resource. 
%\hl{For workloads SSJoin and decompress, their performance is not affected 
%by the data access latency significantly. This is expected as they are compute-bound.}


\subsection{Impact of Computing Capability}
\label{subsec:computing}
As we exploit embedded processors to run in-storage applications, 
it will be interesting to understand how the in-storage 
computing capability affects the efficiency of IceClave. 
%that more performance 
%benefit will come from more powerful embedded cores. 
We vary this parameter by using various models of embedded processor. We use our in-storage computing simulator to simulate 
the representative out-of-order (OoO) ARM processor A72, and the in-order processor A53 with different frequencies. 
We compare IceClave with the baseline Host that has an Intel i7-7700K processor running at 4.2GHz. 

We show the normalized speedup in Figure~\ref{fig:core_ipc}. The performance of IceClave drops 13.7--33.4\%
as we decrease the CPU frequency of ARM processors. And an OoO processor A72 performs slightly better than the in-order processor 
A53 with the same CPU frequency. This demonstrates that IceClave can work with different type of ARM processors and deliver 
reasonable performance benefits. 

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth, trim={0 0.3cm 0 0},clip]{figures/lat.pdf}
	\vspace{-3.8ex} 
	\caption{IceClave outperforms host-based computing for I/O-intensive workloads, as we vary the flash device latency.}
	\label{fig:lat}
		\vspace{-3ex}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/core_ipc.pdf}
	\vspace{-5.5ex} 
	\caption{Sensitivity analysis of IceClave, as we vary the in-storage computing capability.
	}
	\label{fig:core_ipc}
		\vspace{-3ex}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/dram.pdf}
	\vspace{-5.5ex} 
	\caption{Sensitivity analysis of IceClave, as we vary the DRAM size in the SSD controller.
	}
	\label{fig:dram-perf}
	\vspace{-3ex}
\end{figure}

\subsection{{Impact of DRAM Capacity in SSD}}
\label{subsec:dram}
{To evaluate the impact of the SSD DRAM capacity on the IceClave performance, we change the SSD DRAM size from 
4GB to 2GB while using the same configurations as described in Table}~\ref{tab:simconfig}. 
{We present the experimental results in Figure}~\ref{fig:dram-perf}. 
{As we decrease the SSD DRAM capacity, the performance of ISC drops by 12\%--44\%, as it has limited memory space to 
store its data set. The performance of IceClave follows the same trend. However, compared to ISC, IceClave still introduces 
minimal performance overhead.  
}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/twoclaves.pdf}
	\vspace{-6ex} 
	\caption{IceClave performance as we run two in-storage applications concurrently.
	}
	\label{fig:twoclaves}
	\vspace{-3ex}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/fourclaves.pdf}
	\vspace{-6ex} 
	\caption{IceClave performance as we run four in-storage applications concurrently.
	}
	\label{fig:fourclaves}
	\vspace{-3ex}
\end{figure}%ssss

\subsection{{Performance of Multi-tenant IceClave}}
\label{subsec:multitenant}
To further evaluate the efficiency of IceClave, 
we run multiple IceClave instances concurrently, and each instance hosts one of the 
in-storage workloads as described in Table~\ref{tab:workload}. 
We compare the application performance with the case of 
running each in-storage application independently without collocating with other instances. 
As shown in Figure~\ref{fig:twoclaves}, when we collocate the TPC-C instance with other 
workloads, the performance of in-storage applications is decreased by 6.1--15.7\%. 
As we increase the number of collocated instances (see Figure~\ref{fig:fourclaves}), 
their performance drops by 21.4\% on average. This is mainly caused by (1) the computational interference 
between the collocated IceClave instances, and (2) the increased cache misses (up to 8.7\%) 
of the cached mapping table in the protected memory region. 
%(which will cause context switches to the secure world for updating the mapping table entries). 
However, these in-storage programs still perform better 
than host-based approaches that are constrained by the external I/O bandwidth of SSDs. 
%As discussed in $\S$~\ref{subsec:overhead}, IceClave introduces minimal performance overhead to 
%in-storage programs, while ensuring their security isolation.  

==> IceClave (arxiv extended abstract)/impact.tex <==
\section{Significance and Long-term Impact}
This work would have a long-term impact on
%the future development of in-storage computing and future research on security for accelerator devices.
the future development and deployment of in-storage computing, and the future research on securing new computing paradigms.

% 1
%\paragraph{(1) Threat Analysis for In-Storage Computing.}
\paragraph{(1) It provides a comprehensive threat analysis for in-storage computing.}
%Although in-storage computing has been intensively developed recently, 
This paper is the first to focus on security threats faced by in-storage computing. 
%Based on our analysis, future works on in-storage computing should also take security into consideration in addition to improving performance and programmability.
We carefully investigated existing in-storage computing systems and discovered several vulnerabilities that may lead to severe consequences: (a) A malicious user can manipulate the intermediate data and output generated by in-storage programs via both software and physical attacks, causing incorrect computing results; (b) A malicious program can intercept FTL functions like GC and wear leveling in the SSD and mangle the flash management, causing data loss or device destroyed; (c) A malicious user can steal user data stored in flash chips via physical attacks.
%	like bus snooping attack, when 
%		in-storage programs load data from flash chips to SSD DRAM.
%We present them as follows: 
%\begin{itemize}[leftmargin=*]
%    \item {A malicious user can manipulate the intermediate data and output generated 
%    	by in-storage programs via both software and physical attacks, causing incorrect computing results. }
%\vspace{0.5ex}
	%\item {A malicious program can 
%		intercept FTL functions like GC and 
%	        wear leveling in the SSD and mangle the flash management. This would cause data loss 
%		or device destroyed. } 
%\vspace{0.5ex}
%	\item {A malicious user can steal user data stored in flash chips via physical attacks 
%	like bus snooping attack, when 
%		in-storage programs load data from flash chips to SSD DRAM. }
%\end{itemize}
%
%Although there is still space for improvement in performance and programmability of in-storage computing,
We have to overcome these security challenges for its widespread deployment, considering they pose severe threats to user data and flash devices.

% 2
%\paragraph{(2) Security Solution for In-Storage Computing.}
\paragraph{(2) It offers a security solution for in-storage computing.}
We investigated the feasibility of applying existing solutions to secure in-storage computing, unfortunately, 
most of them do not work properly and efficiently with in-storage computing.
For example, we can develop an OS, a hypervisor, or a SGX-like solution for in-storage computing. However, due to the limited resources  
in the SSD controller, they introduce significant overheads to the SSD and increase the attack surface, due to their large codebases. 
%We can also adopt SGX-like solutions. 
%However, this requires significant hardware changes in modern SSDs. 
%As SGX was developed as a generic framework for host machines, it is hard to achieve optimal performance for 
%in-storage programs.
%Moreover, these techniques are not sufficient to defend against the aforementioned attacks.
%An alternative solution is to enable computation on encrypted data~\cite{opaque:nsdi17}. 
%However, such an approach requires intensive compute resource, which cannot be satisfied by modern SSD controllers, due to the resource limits~\cite{biscuit}. 

We proposed the first trusted in-storage computing framework that takes security as the priority. We demonstrated the necessity and feasibility of incorporating the unique flash properties and in-storage workload characteristics into the design for achieving strong security and decent performance at the same time. Our evaluation shows that the performance and hardware cost of IceClave are acceptable for real production systems. 
We believe that security will become a standard feature for computational storage devices, and storage vendors can use IceClave as a reference for building secure computational SSDs.

% 3
%\paragraph{(3) New Memory Encryption and Verification Scheme.}
\paragraph{(3) It develops a new memory encryption and verification scheme.}
IceClave proposes to use hybrid encryption counters for different memory access patterns. While we apply this technique to exploit the fact that in-storage computing workloads are read-intensive, the same idea can be generalized to other systems if we know the workload characteristics. IceClave will inspire future work on memory encryption and verification schemes for applications with different memory access patterns.

% 4
% IceClave inspires TEE for new computing paradigms
% accelerator-centric, in-network computing, etc.
%\paragraph{(4) Implication on New Computing Paradigms.}
\paragraph{(4) It has implications on new computing paradigms.}
As different computing paradigms (e.g., in-storage/in-memory computing, and accelerator-centric computing) offer different execution environments and have their unique architecture and security challenges, it is not easy to apply a TEE solution from one domain to another. This is also true as we shift from host-based computing to in-storage computing, especially with the goal of achieving both efficiency and enhanced security. We believe that IceClave will inspire the development of TEEs for these new computing paradigms. For example, we expect that a TEE framework would be built for securing accelerators. 
%as more applications, especially those AI-based ones, are deployed on hardware accelerators.
%a general TEE framework would simplify the development effort for securing accelerators, and IceClave would inspire the development of this research direction.

% 5
%\paragraph{(5) Deployment in Multi-Tenant Clouds.}
\paragraph{(5) It facilitates the deployment of computational storage in multi-tenant clouds.}
Computational storage devices are becoming more pervasive in clouds. %~\cite{Torabzadehkashi2019ComputationalSA}.
Although TEEs have already been deployed for the host machines in the cloud, there is no support for in-storage TEEs, 
which poses significant security threats to sensitive user data.
IceClave is developed based on a realistic threat model for multi-tenant clouds and is well-suited for this scenario.

% 6
%\paragraph{(6) Deployment in Edge IoT Systems.}
\paragraph{(6) It enables the secure deployment of computational storage in edge IoT systems.}
As computational storage is being widely deployed in edge IoT systems~\cite{aws_greengrass_ngd},
they suffer from physical attacks~\cite{iot_physical_attacks}. Since these devices are often deployed in the public or wild fields, it is extremely easy for an attacker to get physical access to IoT devices. The attacker can unsolder the device and steal data from the flash memory, and tamper with the storage controller to cause unintended behaviors.  
%or eavesdrop the communication between the IoT device and the cloud. Even worse, security vulnerabilities in edge devices can become attack vectors to compromise the cloud server that communicates with these IoT devices. 
The limited hardware resource and power budget of edge devices introduce even more challenges for securing the computational storage.
IceClave is a lightweight solution that can protect computational storage against physical attacks, without introducing much overhead to the resource-limited edge devices.

% \textbf{Ransomware Attacks and In-Storage Forensics.}
% IceClave provides a trusted execution environment that protects the SSD firmware against malware and physical attacks.
% As existing works have exploited the SSD firmware to perform automatic backup and conduct storage forensics [CITATION],
% % TODO: cite TimeSSD, etc.
% the security guarantees provided by IceClave can further enhance the reliability of backup functionalities and the trustworthiness of forensic results.

% 7
%\paragraph{(7) Flexibility of IceClave Implementations.}
\paragraph{(7) It provides the implementation flexibility for different processor architectures.}
IceClave leverages ARM TrustZone to enable the memory protection between 
in-storage programs and FTL functions. This is driven by the fact that ARM processors are available in a majority of 
modern SSD controllers. 
%As device vendors are also considering adopting the open-source RISC-V architecture in their 
%controllers~\cite{riscv-samsung}, 
The key idea of IceClave can also be implemented with new type of processors. 
For instance, RISC-V defines three levels of privileges. We can map the normal, protected, and secure memory regions to different memory regions in RISC-V.
Beyond ARM and RISC-V processors, 
recent works also deployed hardware accelerators in SSD controllers~\cite{biscuit}. 
They are also lacking the in-storage TEEs. We believe IceClave will also facilitate the TEE development for in-storage accelerators.

% TODO: impact on storage industry
% \paragraph{Impact on Storage Industry.}
% TODO: how will IceClave affect how SSD manufacturers design future storage devices?

% \paragraph{Citation for the Test of Time award.}
% This paper is the first to comprehensively characterize and address the security problems of in-storage computing. It presented the first trusted execution environment for in-storage computing with low performance and hardware cost, and laid the foundation for the secure deployment of computational storage in a variety of computing platforms.

==> IceClave (arxiv extended abstract)/implt.tex <==

\begin{table}[t]
    \centering
    \caption{Computational SSD simulator.}
    \vspace{-2ex}
    \footnotesize
    \label{tab:simconfig}
    \begin{tabular}{|l|l|}
        \hline
    	\textbf{SSD Processor}             & ARM Cortex-A72 1.6GHz{~\cite{www:smartssd,arm:storage}}                                  \\ \hline
        Decoder Width         & 3 ops                                                                                                 \\
        Disp/Retire Width & 5 ops \\                                                                          
        L1 I/D Cache          & 48KB/32KB                                                                                             \\
        L2 Cache              & 1MB                                                                                                 \\ \hline
        \textbf{SSD DRAM}  & DDR3 1600 MHz  \\ \hline              
        %	& \begin{tabular}[c]{@{}l@{}}4GB\\ 1 Channel\\ 2 Ranks/Channel\\ 8 Banks/Rank\end{tabular} \\ \hline
        	Capacity & 4GB \\
        	Organization & 1 Channel, 2 Ranks/Channel, 8 Banks/Rank \\
        	Timing & $t_{RCD}$-$t_{RAS}$-$t_{RP}$-$t_{CL}$-$t_{WR}$ = 11-28-11-11-12 \\
        %	Counter Cache:         & 128KB, 8-way, 64B lines, LRU                                                                          \\ 
        	Encryption Delay      & AES-128: 60ns                                                                                         \\ \hline
        \textbf{SSD}  & 1TB Flash-based SSD \\ \hline   
        	%Organization & 32 channels, 4 chips/channel, 8 planes/chip \\ 
        	%& 512 blocks/plane, 128 pages/block, 16KB/page \\ 
        	%Latency & 53$\mu$s for flash array access \\
        	%Bandwidth & 800 MB/s per channel \\ \hline
        	Organization & 8 channels, 4 chips/channel, 4 dies/chip \\
        	& 2 planes/die, 2048 blocks/plane \\
        	& 512 pages/block, 4KB page\\
        	& $t_{RD}$/$t_{WR}$=50/300$\mu$s\\
        	Bandwidth & 600 MB/sec per channel \\
    	\hline	
    \end{tabular}
    	\vspace{-2ex}
\end{table}


\section{Implementation Details}
\label{sec:implt}

\noindent
\textbf{Full System Simulator.}
We implement IceClave with a computational SSD simulator developed based on the
SimpleSSD~\cite{simplessd}, Gem5~\cite{gem5}, and USIMM~\cite{usimm} simulator.
This allows us to conduct the study with different SSD configurations, which cannot be 
easily conducted with a real SSD board. 
We use the SimpleSSD to simulate a modern SSD and its storage operations. 
We show the  
SSD configuration in Table~\ref{tab:simconfig}. 
%We assume a flash array access
%latency of 53$\mu$s, 16 channels, 4 flash chips per channel, 8 planes per chip, 512 blocks per plane,
%and 128 pages per block. Each flash page is 16KB in size and each flash channel has a bandwidth of 
%800MB/s~\cite{micronflashdiesize}.
To enable in-storage computing in the simulator, we utilize Gem5 to model the 
out-of-order ARM processor in the SSD controller. %(see the in-storage processor in Table~\ref{tab:simconfig}). 
%As discussed in $\S$~\ref{subsec:encryption}, 
We also implement the stream cipher in the integrated 
simulator to enable the data encryption/decryption as in-storage applications load data from flash chips. 
We use CACTI 6.5~\cite{cacti} to estimate its hardware cost, and find that the cipher engine introduces 
only 1.6\% area overhead to a modern SSD controller such as that of Intel DC P4500 SSD. 

As IceClave will enable the memory verification in SSD DRAM, we leverage USIMM to
simulate the DRAM in the SSD. We implement the Bonsai Merkle Tree (BMT) in the USIMM simulator, and 
use the hybrid-counter mode (see $\S$\ref{subsec:memory}) as the memory encryption scheme.
As discussed, the root of the integrity tree is stored in a 
secure on-chip register. The counter cache size is 128KB. %We use a 128KB cache for caching counters.
To enable memory encryption and integrity verification, we enforce that each memory access will  
trigger the verification and update of the MAC and integrity tree. 
As we develop a full system simulator with Gem5, we run real data-intensive workloads, such as 
transaction database to evaluate the efficiency of IceClave in the following section.  
%We use a 128KB dedicated metadata cache for caching counters.  
%We compare our proposed design: SC-128, following the split-counter scheme~\cite{encryption:isca06} against the a non-secure system and a SC-64 scheme, to illustrate the performance overhead imposed by our scheme.

\begin{figure}[t]
        \centering
        \includegraphics[width=0.85\linewidth]{figures/cipher_design-v2.pdf}
        \vspace{-2ex}
        \caption{Stream cipher engine design in IceClave.
        }
        \label{fig:cipher_design}
        	\vspace{-2ex}
\end{figure}


\noindent
\textbf{Real System Prototype.}
%In our simulator, we implement IceClave runtime using C progrmaming language. 
{To verify the core functions of IceClave, including TEE creation/deletion, FTL, and stream cipher engine, 
we also implement IceClave with an OpenSSD Cosmos+ FPGA board} that has a Dual ARM Cortex-A9 
processor~\cite{openssd-web}. We measure their overheads and show them in Table~\ref{tab:overhead}. 
%IceClave runtime will create a TEE when an application is offloaded to the SSD, and delete the 
%TEE when the offloaded in-storage application is completed or terminated. 
We demonstrate the architecture of the stream cipher engine in Figure~\ref{fig:cipher_design}.
Its key initialization block takes a symmetric key and an arbitrary initialization vector (IV) as the input
to initialize the cipher. IceClave keeps the key in a secure register, while the IV can be public.
Once initialized, the stream cipher generates 64 keystream bits per cycle.
The generated keystream is XORed bitwise with the data read from flash chips to produce the ciphered data.
%On the other side,
The decipher uses the same key and IV to decode the ciphered data.
%The IV needs to be unique during the entire process for security.
The IV is constructed with temporally unique random numbers and spatially unique address bits.
The orthogonal uniqueness enforces a strong guarantee that the same IV value will not be used twice 
during a certain period of time.
The stream cipher algorithm we used refers to the Trivium~\cite{Trivium}.
{To provide the uniqueness for different flash pages, we compose the IV by concatenating its physical page
address (PPA) and the output of a pseudo-random number generator (PRNG). }
%We implement the stream cipher engine in the SSD controller as follows.  %following the Trivium-64 scheme~\cite{Trivium, triadv1}. 
%It reads 288 state bits from the state register, produces 64 keystream bits, and generates 288 next-state bits.
%%Prior work~\cite{triadv1} reports a consumption of 3051 Gates Equivalent (GE) and 128.7$\mu$W. 
%%According to the energy modeling in~\cite{triadv1}, it takes only 10.3nJ to encrypt a 4KB flash page.
%Moreover, the stream cipher engine introduces minimal area overhead (1.6\% of the entire SSD controller) to a commodity SSD~\cite{flashctrl:fms17, onfi3:fms14}.
%


%To evaluate the performance of our design, we conduct cycle-accurate simulations with workloads from four essential database operations and benchmark suites: TPC-H. These workloads are described in Table x, along with their write ratio. We generate the memory traces for these workloads with PIN ~/cite{Pin}: the traces are generated for 1 billion memory accesses after fast-forwarding to the region of interest. These traces are then fed into cycle-accurate memory system simulator USIMM ~\cite{usimm}. USIMM parameters are listed in ~\tabref{tab:simconfig}, simulating a single-core Out-Of-Order ARM processor.




==> IceClave (arxiv extended abstract)/introduction.tex <==
\section{Introduction}
\label{sec:intro}
In-storage computing has been a promising technique for accelerating data-intensive 
applications, especially for large-scale data processing and analytics~\cite{biscuit}. 
It moves computation closer to the data stored in the storage devices like  
flash-based solid-state drives (SSDs), such that it can overcome the  
I/O bottleneck by reducing the amount of data transferred between 
the host machine and storage devices. 
As modern SSDs are employing multiple general-purpose embedded processors 
and large DRAM in their controllers, it becomes feasible to enable in-storage 
computing in reality today. 

To facilitate the wide adoption of in-storage computing, a variety of frameworks have 
been proposed.
All these prior works show the great potential of in-storage 
computing for accelerating data processing in data centers. 
However, most of them focus on the performance and programmability, but few of them treat the security as the first 
citizen in their design and implementation, which imposes great threat to the user data and 
SSD devices, and further hinders its widespread adoption.

As in-storage processors operate independently from the host machine, and modern  
SSD controllers do not provide a trusted execution environment (TEE) for programs running inside the SSDs,  
they pose severe security threats to user data and flash chips. 
To be specific, a piece of offloaded (malicious) code
could (1) manipulate the mapping table in the flash translation layer (FTL) to mangle  
the data management of flash chips, (2) access and destroy data belonging 
to other applications, and (3) steal and modify the memory of co-located 
in-storage programs at runtime. Even worse, adversaries can steal and modify intermediate data and results generated by in-storage programs via physical attacks such as cold-boot attack, bus snooping attack, and replay attack~\cite{physicalattack:blackhat2014}.  

To overcome these security challenges, state-of-the-art in-storage computing frameworks maintain a copy of the privilege information in the SSD DRAM and enforcing permission checks for in-storage programs.
However, such a solution still suffers from many security vulnerabilities~\cite{sok}.
An alternative approach is to adopt Intel SGX.
Unfortunately, modern in-storage processors do not support SGX,
and it also incurs significant performance overhead~\cite{www:intelsgx}.

% To overcome these security challenges, there are existing TEE frameworks such as Intel SGX.
% Unfortunately, modern in-storage processors do not support SGX, and it also incurs significant performance overhead, which cannot be afforded by SSD controllers.

Therefore, providing a secure, lightweight, and trusted execution environment for in-storage computing 
is an essential step towards its widespread adoption. 
Ideally, we wish to enjoy the performance benefits of in-storage computing, while 
enforcing the security isolation between in-storage programs, the core FTL functions, and physical 
flash chips, as demonstrated in Figure~\ref{fig:goals}.  

To this end, we present IceClave, a trusted execution environment for in-storage computing. 
IceClave is designed specifically for modern SSD controllers 
and in-storage programs, with considering the unique flash properties and in-storage workload characteristics. 
With ensuring the security isolation, IceClave includes (1) a new memory protection scheme to protect the FTL and reduce the context switch overhead 
incurred by flash address translations; (2) a technique for securing in-storage DRAM for in-storage programs by taking 
advantage of the fact that most in-storage applications are read intensive; (3) a stream 
cipher engine for securing data transfers between storage processors and flash chips, with low performance overhead and energy consumption; 
and (4) a runtime system for managing the life cycle of in-storage TEEs.

\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{./figures/goals-v1.pdf}
\vspace{-1.5ex}
\caption{IceClave enables in-storage TEEs to achieve security isolation between in-storage programs, 
	FTL, and flash chips.}
\label{fig:goals}
\vspace{-3.5ex}
\end{figure}

We implement IceClave with a full system simulator
and develop a real system prototype with a real-world OpenSSD Cosmos+ FPGA board.
Compared to state-of-the-art in-storage computing approaches,  
IceClave introduces only 7.6\% performance overhead to the in-storage runtime
and delivers 2.31$\times$ better performance than host-based computing,
while adding minimal area and energy overhead to the SSD controller. 

==> IceClave (arxiv extended abstract)/relatedwork.tex <==
\section{Related Work}
\label{sec:related}

\textbf{In-storage Computing.}
In-storage computing has been intensively developed recently. 
Researchers have been exploring it for applications such as
database query~\cite{summarizer,Do:2013:QPS:2463676.2465295,kang2013enabling,smartssd},
key-value store~\cite{willow}, map-reduce workloads~\cite{biscuit,kang2013enabling},
signal processing~\cite{ActiveFlash}, and scientific
data analysis~\cite{Tiwari:2013:AFT:2591272.2591286,Tiwari:2012:RDM:2387869.2387873}.
%They %treat the SSDs as compute device and leverage the embedded CPU processors
%utilize the embedded processors in the SSD controller
%to perform computing operations, such that it can move computation closer to the data for 
%avoiding large amount data transfer over PCIe. 
To enable in-storage computing in modern SSDs, 
these prior works have developed various frameworks~\cite{biscuit,willow,summarizer,insider:atc19}. 
However, most of them focus on the 
programmability and performance. %without paying much attention on the in-storage security. 
Although there is still space for improvement in these aspects, such as having SSD array and filesystem  
support for in-storage computing{~\cite{insider:atc19}}, we have to overcome the security challenge of in-storage computing for its widespread deployment, since it poses threats to user data and flash devices.
%As in-storage computing is being widely deployed in practice~\cite{samsungsmartssd, scaleflux}, 
%it poses threats to user data and storage devices. 
To the best of our knowledge, we are the first to propose building trusted execution environments for in-storage computing.  
%propose building trusted execution environments for in-storage computing. 
%To the best of our knowledge, we are the first 
%to propose building trusted execution environments for in-storage computing. 
%To the best of our knowledge, 
%we are the first to propose building trusted execution environments for in-storage computing. 

\textbf{Trusted Execution Environment.}
To defend applications from malicious systems software, trusted hardware  
devices have been developed. A typical example is Intel SGX~\cite{haven}, which can create 
trusted execution environments for applications. 
{Because of the enabled security isolation, SGX is extended or customized 
to support various computing platforms}~\cite{graviton:osdi2018, scone:osdi2016, obliviate, pesos:eurosys2018, sanctum:usenixsec2016} {and 
applications}~\cite{vc3:oakland2015, enclavedb, shieldstore:eurosys2019, speicher:fast2019}. 
The hardware devices with TPM~\cite{tpm} serve the similar purpose by utilizing 
the attestation available in commodity processors from AMD and 
Intel~\cite{flicker,logicalattestation,trustvisor}. 
For ARM processors that are commonly used in 
mobile devices and storage controllers, they offer TrustZone that enables users 
to create secure world isolated from the OS~\cite{vtz, trustzone:asplos14}. Unfortunately, none of these hardware devices can be directly applied 
to in-storage computing. %and defend against physical attacks. 
%{For instance, %Guardat}~\cite{guardat:eurosys2015} {and Pesos}~\cite{pesos:eurosys2018} {allow 
%users to specify security policies in storage devices to protect data confidentiality and integrity, 
The most recent work 
ShieldStore~\cite{shieldstore:eurosys2019} {and Speicher}~\cite{speicher:fast2019} {applied SGX to key-value stores, however, none of them can protect 
the execution of in-storage programs.} 
We develop specific trusted execution environments for in-storage applications. 
%for security isolation with minimal hardware cost. 

\textbf{Storage Encryption and Security.} 
As we move computation closer to data in the storage devices, it would inevitably increase 
the trusted computing base, which poses security threats to user data. To protect sensitive user 
data while enabling near-data computing, a common approach is data encryption~\cite{denfs}. 
However, data leakage 
or loss would still happen at runtime, due to the lack of TEE support in 
modern SSD controllers. And adversaries can also initiate physical attacks to steal/destroy user data. 
An alternative approach is to enable computation on encrypted data~\cite{opaque:nsdi17, ocq:eurosys2020}. 
However, such an approach requires 
intensive computing resource, which cannot be satisfied by modern SSD controllers due to the 
limited resource budget~\cite{deepstore:micro2019, neardata, biscuit, timessd:eurosys2019}. 
Our work IceClave presents a lightweight approach that can enforce security isolation for in-storage 
applications as well as defend against physical attacks. 


==> IceClave (arxiv extended abstract)/runtime.tex <==
\subsection{IceClave Runtime}
\label{subsec:runtime}
In this section, we discuss how IceClave runtime facilitates the execution of in-storage TEEs. 
%IceClave runtime is developed based on the ARM TrustZone with the security techniques we discussed in previous sections.  
It provides the essential functions for managing in-storage TEEs, such as TEE setup, TEE lifecycle 
and metadata management, and the interaction with the secure world. 
%It is the software measure that extends our proposed security features for in-storage-computing based on ARM TrustZone. 
IceClave runtime also interacts with IceClave library deployed in the host machine. Note that 
IceClave library only exposes basic offloading interfaces (e.g., RPC) to end users. 
This not only reduces the trusted computing base but also simplifies the development of in-storage programs. 
We list the APIs of IceClave in Table~\ref{tab:api}. 

IceClave allows a user to interact with the SSD using two APIs: \texttt{OffloadCode} and \texttt{GetResult}. 
Once the program is offloaded to the SSD, IceClave runtime will execute \texttt{CreateTEE()} to create 
a new TEE. %Upon successful return, the TEE is initialized and gets an TEE ID. 
At the same time, 
it will call \texttt{SetIDBits()} to set the ID bits (access permission, see $\S$\ref{subsec:mapping}) 
of the corresponding address mapping table entries in FTL with the list of logical page addresses specified 
by the in-storage program. According to our study on the popular in-storage programs, their code size 
is 28--528KB. However, for an offloaded program whose size is larger than the available space of SSD DRAM, 
the TEE creation will fail.
During the execution of an in-storage program, \texttt{ThrowOutTEE()} will be called to handle program 
exceptions. IceClave runtime will abort the TEE for these cases that include (1) access control is violated, 
(2) TEE memory or metadata is corrupted, and (3) in-storage program throws an exception.
Once the in-storage program is finished, IceClave runtime will call the \texttt{TerminateTEE()} to terminate 
the TEE. %reclaim its allocated memory, and its TEE ID. %Once this is performed, the TEE can no longer be accessed via any means.
%We will describe the detailed workflow in the following section. 

With the assistance of TrustZone, IceClave supports dynamic memory allocation within each TEE. To avoid 
memory fragmentation, IceClave will preallocate a large contiguous memory region (16MB by default). Upon 
TEE deletion, IceClave runtime will release the preallocated memory region.



==> IceClave (arxiv extended abstract)/threatmodel.tex <==
\section{\NoCaseChange{Threat Model}}
\label{sec:threatmodel}
We target the multitenancy where multiple application instances operate in the shared 
SSD. Following the threat models for cloud computing today,
we assume the cloud computing platform has provided a secure channel for end users to offload 
their programs to the shared SSD. The related code-offloading techniques, such as secure RPC and libraries, have already been deployed in cloud platforms~\cite{f1}. 
However, an offloaded program can include (hidden) malicious code.

We assume hardware vendors do not intentionally implant backdoor or malicious programs in their 
devices. However, as we deploy those computational SSDs in shared platforms (e.g., public cloud), 
we do not trust the platform operators who could initiate board-level physical attacks such as 
bus-snooping and man-in-the-middle attacks, or exploit the host machine to steal or destroy data 
stored in SSDs. Similar to the threat model for SGX, 
we assume that the processor chip is safe against physical attacks, and we exclude software side-channel attacks~\cite{www:intelsgx}.

==> abstract.tex <==
\begin{abstract}
In-storage computing with modern solid-state drives (SSDs)   
enables developers to offload programs from the host to the 
SSD. It has been proven to be an effective approach to alleviating the I/O bottleneck. 
To facilitate in-storage computing, many frameworks have been proposed. 
However, few of them treat the 
in-storage security as the first citizen. 
Specifically, since modern SSD controllers do not have a trusted execution environment, 
an offloaded (malicious) program could steal, modify, and even destroy the data stored in 
the SSD. 

In this paper, we first investigate the attacks that could be conducted by offloaded in-storage 
programs. To defend against these attacks, we build a lightweight trusted
execution environment, named IceClave for in-storage computing. 
IceClave enables security isolation between in-storage programs and flash management functions.  
IceClave also achieves security isolation between in-storage programs and enforces
memory encryption and integrity verification of in-storage DRAM with low overhead. To protect data loaded from flash chips,   
IceClave develops a lightweight data encryption/decryption mechanism in flash controllers.  
We develop IceClave with a full system simulator. 
We evaluate IceClave with a variety of 
data-intensive applications such as databases.
Compared to state-of-the-art in-storage computing approaches, 
IceClave introduces only 7.6\% performance overhead, while enforcing security isolation in 
the SSD controller with minimal hardware cost.  
IceClave still keeps the performance benefit of in-storage computing by delivering up to 2.31$\times$
better performance than the conventional host-based trusted computing approach.

\end{abstract}


==> ack.tex <==
\begin{acks}
We thank the anonymous reviewers for their comments and feedback. This work was 
partially supported by NSF grant CNS-1850317 and CCF-1919044, a gift fund from SK Hynix, and the Department of Defense under Contract FA8075-14-D-0002-0007, TAT 15-1158.
\end{acks}

==> alltogether.tex <==
\subsection{Put It All Together}
\label{subsec:all}


We illustrate the entire workflow of running an in-storage program with IceClave in Figure \ref{fig:workflow}. 
%The end users rely on IceClave library to offload their programs to the shared SSD. 
Similar to existing in-storage computing frameworks~\cite{willow, biscuit}, IceClave library 
has a host-to-device communication layer based on PCIe, which allows users to transfer data between 
the host and SSD. As discussed in {$\S$\ref{sec:threatmodel}}, we utilize the secure channel developed in 
modern cloud computing platforms for interactions between the host and shared SSD.
%The \texttt{OffloadCode} API (\circlep{1}) described in $\S$\ref{subsec:runtime} is called 
The \texttt{OffloadCode} API (\circlep{1}) described in $\S$\ref{subsec:runtime} is called to offload programs. 
Its parameter \texttt{bin} represents the pre-compiled program in the form of machine code, and
\texttt{lpa} is a list of Logical Page Addresses (LPAs) of data needed by the offloaded program.
It uses task ID (\texttt{tid}) as an index for identifying the offloaded procedure.

IceClave runtime will create a new TEE for the offloaded program using \texttt{CreateTEE} ({\circlep{2}}). 
At creation, IceClave runtime will allocate memory pages from the normal memory region to the TEE, while 
the TEE metadata will be initialized and maintained in the secure memory region. IceClave also executes  
\texttt{SetIDBits} to set access permissions in the address mapping table for {LPAs}. 
%specifying page table address, program identity and other security info. 
%The user program binary will be copied into the TEE after the TEE is successfully initialized.     
The TEE does not rely on FTL to get physical page addresses (see $\S$\ref{subsec:ftl}),  
as it can access the mapping table in the protected memory region (\circlep{3}). 

However, the in-storage program may occasionally encounter cache misses, when a mapping entry for the accessed 
LPA is not cached in the SSD DRAM. In this case, the TEE has to redirect the address translation request 
to the FTL via \texttt{ReadMappingEntry} (\circlep{4}). This TEE will be paused and switched to the secure world, such 
that FTL will load the missing mapping table pages (\circlep{5}), update the cached mapping table in the protected memory 
region, and return the PPA to the TEE. To avoid in-storage programs probing the entire physical space 
of the SSD, we enforce the access control (see $\S$\ref{subsec:mapping}). 
Any data on the data path to the TEE is encrypted with the stream cipher engine (\circlep{6}). Note that 
users are encouraged to encrypt their data to defend against attacks from malicious host OS. They will send their decryption key to 
the TEE along with the offloaded program, and decrypt the data at runtime in the TEE. 
%Above security enforcement measures are managed automatically by IceClave without user notice.
\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/workflow.pdf}
	\vspace{-2ex}
	\caption{IceClave workflow of running in-storage programs. In this diagram, IceClave Runtime and Library, TEE, FTL, Stream Cipher Engine, and Flash Controller are compute regions. Mapping Table and Flash are memory regions.
	}
	\label{fig:workflow}
		\vspace{-3ex}
\end{figure}
The TEE will be invoked by IceClave runtime once the in-storage program is readily prepared inside the TEE. 
IceClave runtime constantly monitors the status of initiated TEEs, secures memory regions, and ensures the 
mapping table permission guard. Exceptions will be thrown out if any aforementioned integrity is compromised. 

During the entire lifecycle of a TEE, the hardware protection mechanisms described in $\S$\ref{subsec:memory} 
are enforced to prevent physical memory attacks. IceClave will also enforce strong isolation between 
TEEs and the FTL. The memory protection described in $\S$\ref{subsec:ftl} will also be enforced in existing 
TrustZone memory controller (TZASC)~\cite{TZASC}. Once reaching the end of the TEE program, 
the results are copied into the TEE's metadata region before terminating the TEE and reclaiming used resources (\circlep{8}). 
IceClave will initiate a DMA transfer request to the host using NVMe interrupts, signaling the readiness of results. 
Results are returned to the host memory via \texttt{GetResult} (\circlep{7}) provided in IceClave library.



==> background.tex <==
\section{Background and Motivation}
\label{sec:motivation}
In this section, we first introduce the background of flash-based SSDs and 
in-storage computing, and discuss why it is desirable to have TEEs 
for in-storage computing. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{./figures/ssdhardware.pdf}
    \vspace{-2ex}
    \caption{Internal architecture of flash-based SSDs.}
    \label{fig:ssd-arch}
    \vspace{-3ex}
\end{figure}


\subsection{Flash-Based Solid-State Drive}
\label{subsec:ssd}

%Flash-based SSDs provide significant performance improvement %up to 5,000$\times$ higher throughput and up to 100$\times$ lower latency
%than conventional hard-disk drives (HDDs), while their price is fast approaching to that of HDDs.
The rapidly shrinking process technology has allowed SSDs to boost their performance
and capacity, which accelerates their adoption in commodity systems such as data 
centers today~\cite{flashblox, flashmap:isca2015, flatflash:asplos2019}.
We present a typical SSD architecture in Figure~\ref{fig:ssd-arch}.
An SSD has three major components: a set of flash memory packages,
an SSD controller having embedded processors with DRAM, and flash controllers~\cite{chen2011essential, 
deepstore:micro2019}. The flash packages are
organized in a hierarchical manner. Each SSD has multiple channels. 
%where each channel can receive and process read/write commands independently. 
Each channel is shared by multiple flash
packages. Each package consists of multiple flash chips. Each chip has multiple planes. Each plane
is divided into multiple flash blocks, each of which consists of multiple flash pages.


Due to the nature of flash memory,
when a free flash page is written once, that page is no longer available for future writes until
that page is erased.
However, erase operation can be performed only at a block %(which has 64 or more pages) 
granularity, which is time-consuming.
Thus, writes are issued to free pages that have been erased (i.e., out-of-place write) rather than
waiting for the expensive erase operation. 
Garbage collection (GC) will be performed later to clean the obsolete data in SSDs.
As each flash block has limited endurance,
it is important for blocks to age uniformly (i.e., wear leveling).
SSDs employ out-of-place write, GC, and wear leveling to overcome the shortcomings
of SSDs and maintain indirections for indexing the logical-to-physical address mapping.
All these are managed by the Flash Translation Layer (FTL) in the SSD controller.



\subsection{In-Storage Computing}
\label{subsec:instorage}
We have long recognized the inefficiency of traditional CPU-centric computing 
for data-intensive applications that need to transfer large amounts of 
data from storage.
The application performance is limited by the low bandwidth of 
PCIe interface between the host and SSD. % such as PCIe.
To tackle this challenge, various in-storage computing 
approaches~\cite{biscuit, summarizer, willow, capi:2014:whitepaper, deepstore:micro2019} have been proposed.
With them, we can process data by exploiting SSD processors and high internal 
bandwidth of flash chips. %without going through the slow I/O interface. 
Their significant performance benefits show that in-storage 
computing is a promising technique. 

However, as in-storage processors operate independently from the host,  
it poses security challenges to the adoption of in-storage computing, especially in 
the multi-tenancy setting where multiple application instances share the physical 
SSD~\cite{multissd:sigmod2014, documentdb:vldb2015, cloudstorage:osdi2012, libra:eurosys2014, 
slo:fast2015, heracles:isca2015}. 



%\subsection{In-Storage Vulnerabilities and Why In-\\Storage TEE}
\subsection{In-Storage Vulnerabilities}
\label{subsec:why}
%As discussed in existing in-storage computing frameworks~\cite{biscuit, willow}, 
When specific code is offloaded to in-storage processors, a copy of the privilege information is transferred and maintained in the DRAM of the SSD controller~\cite{biscuit,willow}. 
Such a solution is developed under the assumption that the offloaded code has already 
known the address and size of the accessed data in advance.
However, %a malicious program can still intentionally access other data regions inside the SSD 
adversaries can exploit in-storage software and firmware vulnerabilities such as 
buffer overflows~\cite{sok, pointerguard:security2003, bufferoverflow},  
and bus-snooping attack~\cite{ssdflaw} to achieve privilege escalation. After that, 
they can conduct various further attacks.  
We present them in the following. 

\begin{itemize}[leftmargin=*]
    \item {A malicious user can manipulate the intermediate data and output generated 
    	by in-storage programs via both software and physical attacks, causing incorrect computing results. }
\vspace{1ex}
	\item {A malicious program can 
		%manipulate the critical data structures (e.g., mapping 
		%table in FTL) stored in the shared SSD DRAM, and 
		intercept FTL functions like GC and 
	        wear leveling in the SSD and mangle the flash management. This would cause data loss 
		or device destroyed. } 
\vspace{1ex}
	\item {A malicious user can steal user data stored in flash chips via physical attacks 
	like bus snooping attack, when 
		in-storage programs load data from flash chips to SSD DRAM. }
		%even destroy the entire SSD by manipulating the core functions in the FTL. }
		\vspace{1ex}
		
\end{itemize}

To defend against these attacks, an alternative solution is to develop an OS or hypervisor for 
in-storage computing. However, due to the limited resources  
in the SSD controller, running a full-fledged OS can introduce significant overheads to the SSD and increase the attack surface, due to its large codebase.
%it is not easy to run an full-fledged OS, while supporting the execution of 
%in-storage programs efficiently. 
Moreover, these techniques are not sufficient to defend against the aforementioned attacks such as 
board-level physical attacks.
As we move compute closer to storage devices, it is highly desirable to have a lightweight execution environment 
for this non-traditional computing paradigm.


Since SSDs were designed with the assumption they are hardware 
isolated from the host and purely used as storage rather than computing, 
modern computing systems do not provide secure runtime environment for in-storage computing.
As discussed in $\S$\ref{sec:intro}, a straightforward approach is to adopt the SGX-like solutions~\cite{www:intelsgx,keystone:eurosys2020}. 
However, this requires significant hardware changes and even replacement of storage processors available in modern SSDs. 
As SGX was developed as a generic framework for host machines, it is hard to achieve optimal performance for 
in-storage programs. 

%ARM processors 
%available in modern SSD controllers provide the TrustZone technique~\cite{trustzone} to enable 
%the creation of secure world 
%and normal world, however, it is unclear whether and how it can be utilized for in-storage computing, and 
%how it should work seamlessly together with the hardware components in SSD controllers.  
%And most importantly, TrustZone cannot defend against physical attacks. 
%Therefore, 
%%as we move computation to the SSD controller, 
%we have to rethink their system design with considering the security as the first citizen. 
%%and develop TEEs for in-storage programs.  




==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
%This paper investigates security vulnerabilities for in-storage computing. 
Due to the lack of TEE support in SSD controllers, 
adversaries can intervene offloaded programs, mangle flash management, steal and destroy user data.
%As we move forward to in-storage computing for practical 
%benefits, we have to address these security challenges.
To this end, %we develop a
we develop IceClave, a
lightweight TEE which enables security
isolation between in-storage programs and flash management.
IceClave can also defend 
against physical attacks with minimal hardware cost.
%With running data-intensive 
%applications, we show IceClave introduces minimal overhead to application performance,  
%while ensuring security guarantees for in-storage computing.
%\hl{Our evaluation shows} IceClave \hl{ensures security guarantees for in-storage computing programs while incurring minimal overhead.}



==> evaluation.tex <==
\section{Evaluation}
\label{sec:eval}
Our evaluation demonstrates that: (1) IceClave introduces minimal performance overhead to in-storage workloads while
enforcing security isolation in SSD controllers ($\S$\ref{subsec:perf} and $\S$\ref{subsec:overhead}); 
%(2) It has minimal negative impact on the energy efficiency of
%in-storage computing ($\S$\ref{subsec:power}); 
(2) IceClave scales in-storage application performance as we increase the internal bandwidth
of SSDs ($\S$\ref{subsec:bandwidth}); 
(3) It can benefit various SSD devices with different access latencies ($\S$\ref{subsec:latency});
(4) IceClave still outperforms conventional host-based computing significantly while offering security isolation, 
as we vary the in-storage computing capability ($\S$\ref{subsec:computing} and $\S$\ref{subsec:dram}); 
(5) IceClave enables concurrent execution of multiple in-storage  
programs with low performance overhead ($\S$\ref{subsec:multitenant}). 

\begin{table}
    \centering
    \caption{In-storage workloads used in our evaluation.}
    \vspace{-2ex}
    \scriptsize
    \label{tab:workload}
    \begin{tabular}{|p{45pt}|p{145pt}|}
    \hline
                \textbf{Workload}   & \textbf{Description} \\ \hline
        Arithmetic & Mathematical operations against data records                                  \\ \hline
        Aggregation& Aggregate a set of values with average operation     \\ \hline
        Filter     & Filter a set of data that matches a certain feature                                        \\ \hline
        %Inner Join & Select rows that have matching values in both tables                                      \\ \hline
        TPC-H Q1   & Query pricing summary involving scan                    \\ \hline
        TPC-H Q3   & Query shipping priority involving join              \\ \hline
        TPC-H Q12  & Query shipping modes and order priority with join                                           \\ \hline
        TPC-H Q14  & Query market response to promotion with join                                                 \\ \hline
        TPC-H Q19  & Query discounted revenue with join and aggregate           \\ \hline
        TPC-B      & Queries in a large bank with multiple branches                                  \\ \hline
        TPC-C      & Online transaction queries in a warehouse center                              \\ \hline
        Wordcount  & Count the number of words in a long text~\cite{biscuit} \\ \hline
    \end{tabular}
    	\vspace{-3ex}
\end{table}


\subsection{Experimental Setup}
\label{subsec:setup}
We evaluate IceClave with a set of synthetic workloads and real-world applications as shown in Table~\ref{tab:workload}.
In the synthetic workloads, we use several essential operators in database system, including arithmetic, aggregation, and filter operations.
As for the real-world applications, we run real queries from the TPC-H benchmark. Specifically, we use TPC-H Query 1,
3, 12, 14, and 19 that include the combination of multiple join and aggregate operations.
In addition to these workloads, we also run write-intensive workloads TPC-B, TPC-C, and Wordcount to 
further evaluate the encryption and integrity verification overhead of IceClave.
%\hl{It is worth noting that SSjoin and Decompress are also computation-intensive workloads, which are not 
%great workload candidates for in-storage computing according to our experiments and previous study}~\cite{summarizer}. \hl{Therefore, we exclude these two workloads when we report the average performance results through the paper.}
In all these workloads, we populate their dataset (tables) to
the size of 32GB, and place them across the channels in the SSD. %We collect traces from the workloads running on the baseline system to evaluate their access patterns.


We compare IceClave with several state-of-the-art solutions. Particularly, we compare IceClave with the Intel SGX available in the host machine, in which we
load the data from the SSD to the host memory and conduct the queries in the SGX. For this setting, we use a real server, which has an Intel {i7-7700K}
processor running at 4.2GHz, 16GB DDR4-3600 DRAM, and 1TB Intel DC P4500 SSD. {For fair comparison, we follow the specification of the Intel DC P4500 SSD
to configure our SSD simulator. We also compare IceClave with current in-storage computing approaches that do not provide TEEs for offloaded programs. }
We list them as follows:

\begin{itemize}[leftmargin=*]
\vspace{1ex}
    \item \textbf{Host}: in which we load data from the SSD to the host memory, and execute the data queries using host processors.
        The host machine and SSD setups are described above.
\vspace{1ex}
    \item \textbf{Host+SGX}: in which we run data queries within the Intel SGX after loading data from the SSD. The version of the
            SGX SDK we use in our experiments is 2.5.101.
\vspace{1ex}
    \item \textbf{In-Storage Computing (ISC):} in which we run data queries with the ARM processors
            in the SSD controller, such that we can exploit the high internal bandwidth of the SSD.
\vspace{1ex}
\end{itemize}

%We use CACTI 6.5~\cite{cacti} to
%estimate energy utilization of the SRAM (including the one used for stream cipher engine) in the 32nm technology node.
%We use the \texttt{itrs-hp} model for SRAMs of the SSD.
%We assume the DRAM energy is 20-pJ/bit~\cite{markhorwitz}. We use the power consumption of flash page
%access in the Intel DC P4500 SSD to calculate the energy consumed by flash accesses.
%We obtain the energy consumption of processor and network-on-chip using McPAT~\cite{mcpat}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/iscvsvanila.pdf}
    \vspace{-3ex}
    \caption{Performance comparison of Host, Host+SGX, ISC, and IceClave (from left to right).
    We show the performance breakdown of each scheme.}
    \label{fig:iscvsvanila}
    	\vspace{-3ex}
\end{figure}




\subsection{Performance of IceClave}
\label{subsec:perf}
We show the normalized performance of running each query benchmark in Figure~\ref{fig:iscvsvanila}.
We use the Host as the baseline, in which we run the query workload with the host machine while 
loading the dataset from the SSD. As shown in Figure~\ref{fig:iscvsvanila}, IceClave outperforms 
Host and Host+SGX by 2.31$\times$ and 2.38$\times$ on average, respectively. This shows that 
IceClave will not compromise the performance benefits of in-storage computing. 
%while ensuring the security isolation inside SSDs. 
As those data query workloads are bottlenecked by the storage 
I/O, the SGX on the host machine (Host+SGX) slightly decreases the workload performance. 
Compared to in-storage computing without security isolation enabled (ISC), IceClave introduces 
7.6\% performance overhead, due to the security techniques used in the in-storage TEE. 
%\hl{For these compute-intensive workloads such as SSJoin and decompress, as we expected, they do 
%not obtain performance benefits from in-storage computing. However, we still show that} IceClave \hl{introduces 
%minimal performance overhead in comparison with ISC.}


To further understand the performance behaviors of IceClave, we also demonstrate the performance 
breakdown in Figure~\ref{fig:iscvsvanila}. As for the Host and Host+SGX schemes, we partition their 
workflow into two major parts: data load and computing time. As we can see, 
Host+SGX incurs 103\% extra computing time on average, caused by the SGX running in the host machine. 
As for the ISC and IceClave schemes, we profile the data load time from flash chips, the computing 
time with in-storage processors, and the overhead caused by the memory encryption and verification 
for IceClave. As shown in Figure~\ref{fig:iscvsvanila}, IceClave and ISC take much less time on loading 
time, as the internal bandwidth of the SSD is higher than its external bandwidth. And they require  
more time (2.47$\times$ on average) to execute the data queries. Compared to ISC, IceClave needs memory 
encryption and verification. 
For write-intensive workloads such as Wordcount, IceClave slightly increases memory encryption overhead. This is because Merkle tree intrinsically supports parallel updates, and our hybrid-counter design preserves this property by default.
However, IceClave still 
outperforms host-based approaches significantly for a majority of in-storage workloads. 
%\hl{For the workloads SSJoin and decompress, they 
%incur more memory writes during their computation procedure, the memory encryption and integrity verification 
%cause more overheads. However, this is less of a concern, as }

\begin{table}[t]
    \centering
	\caption{Overhead source of IceClave.}
	\vspace{-2ex}
    \footnotesize
    \label{tab:overhead}
	\begin{tabular}{|p{78pt}<{\raggedleft}|p{55pt}<{\raggedright}|}
        \hline
    	\textbf{Overhead Source}   & \textbf{Average Time} \\ \hline
        TEE creation &  95~$\mu$s                                 \\ \hline
        TEE deletion &   58~$\mu$s   \\ \hline
        Context switch    &  3.8~$\mu$s           \\ \hline
        Memory encryption   &    102.6~ns              \\ \hline
        Memory verification   &  151.2~ns             \\ \hline
    \end{tabular}
    	\vspace{-3ex}
\end{table}

\begin{table}[t]
	\centering
	\footnotesize
	\caption{Extra memory traffic caused by memory encryption and verification when running in-storage workloads.}
	\vspace{-2ex}
	\label{tab:memtraffic}
	\begin{tabular}{|c|c|c|}
		%\toprule
		\hline
		\textbf{Workload} & \textbf{Encryption} & \textbf{Integrity Verification}\\ 
		\hline
 		Arithmetic & 3.05\% & 2.27\% \\
 		\hline
		Aggregate & 3.06\% & 2.26\% \\
		\hline
		Filter & 3.04\% & 2.26\% \\
		\hline
		TPC-H Query 1 & 2.99\% & 2.22\% \\
		\hline
		TPC-H Query 3 & 5.62\% & 4.5\%\\
		\hline
		TPC-H Query 12 & 5.11\% & 3.78\% \\
		\hline
		TPC-H Query 14 & 10.28\% & 5.39\%\\
		\hline
		TPC-H Query 19 & 36.20\% & 24.75\%\\
		\hline
		TPC-B & 46.92\% & 36.68\%\\
		\hline
		TPC-C & 39.09\% & 31.72\%\\
		\hline
		Wordcount & 67.45\% & 43.81\%\\
		\hline
% 		\hline
% 		Arithmetic & 10.3\% & 17.3\% \\
% 		\hline
% 		Aggregate & 9.5\% & 16.6\% \\
% 		\hline
% 		Filter & 9.3\% & 16.4\% \\
% 		\hline
% 		TPC-H Query 1 & 9.9\% & 15.4\% \\
% 		\hline
% 		TPC-H Query 3 & 22.4\% & 34.4\%\\
% 		\hline
% 		TPC-H Query 12 & 20.9\% & 28.5\% \\
% 		\hline
% 		TPC-H Query 14 & 46.7\% & 64.5\%\\
% 		\hline
% 		TPC-H Query 19 & 69.7\% & 81.0\%\\
% 		\hline
% 		TPC-B & 39.6\% & 53.4\%\\
% 		\hline
% 		TPC-C & 37.4\% & 49.6\%\\
% 		\hline
	\end{tabular}
		\vspace{-5ex}
\end{table}



\subsection{Overhead Source in IceClave}
\label{subsec:overhead}
We also profile the entire workflow of running an in-storage program with IceClave.  
We show the critical components of IceClave and their overhead in Table~\ref{tab:overhead}. 
IceClave takes 95~$\mu$s and 58$~\mu$s (measured in real SSD FPGA board) to create and 
delete a TEE inside SSD, respectively. The overhead of context switch between 
secure world and normal world is 3.8~$\mu$s. As discussed in $\S$\ref{subsec:ftl}, 
IceClave has infrequent context switches at runtime, as it places the frequently accessed 
address mapping table in the protected memory region. The context switch happens mostly because 
the mapping table entries are missing in the protected memory region, and IceClave needs to switch 
to the secure world to fetch the mapping table from flash chips, and update 
them in the protected memory region. 

Moreover, IceClave incurs much less memory encryption and verification operations, 
because most in-storage workloads are read intensive (see $\S$\ref{subsec:memory} and Table~\ref{tab:memfootprint}). 
The average execution times of each memory encryption and verification take 102.6~ns and 151.2~ns, respectively.  
%To understand the memory overhead of IceClave, 
We profile the additional memory accesses (see Table~\ref{tab:memtraffic}) 
incurred by fetching and overflowing counters in the memory encryption and integrity verification. 
%Table~\ref{tab:memtraffic} shows 
%the increase of memory traffic caused by memory encryption and integrity verification in percentage, compared to 
%the data traffic. 
We show the extra memory traffic in percentage in Table~\ref{tab:memtraffic}, when comparing to the regular memory traffic without 
enforcing memory security. 
Memory encryption and verification increase the memory traffic by 20.26\% and 14.51\% on average, respectively. 

We also profile the number of flash address translations requested from a TEE, and find that only 0.17\% of these address 
translations are missed in the cached mapping table in the protected memory region. This indicates that in-storage programs do not incur the context 
switch from the normal world to the secure world frequently, showing that IceClave is lightweight for in-storage 
workloads.  


%\subsection{Impact on Power Consumption}
%\label{subsec:power}
%We now evaluate the energy efficiency of IceClave against ISC. 
%%We measure the power consumption of the host processors using an open-source tool CPU %Energy Meter~\cite{powermeter} and \textit{perf}~\cite{rapl}.
%With the measurement methods described in $\S$\ref{subsec:setup}, 
%we collect the energy consumption of the entire SSD, including the energy consumed by embedded processors, SSD DRAM, and 
%flash chips. We present the results in Figure~\ref{fig:energy}. 
%Compared to ISC without security isolation,    
%IceClave introduces up to 11.8\% energy overhead. %as we run various query workloads. 
%
%To further understand the energy consumption of IceClave, we show the energy breakdown of all these schemes in 
%Figure~\ref{fig:energy}. It includes the energy consumption of ARM processor, SSD DRAM, and flash access. %and stream cipher engine. 
%Compared to ISC, the energy overhead of IceClave is mainly caused by the extra operations generated by 
%the memory encryption and verification. The stream cipher engine of IceClave adds trivial energy overhead (0.01\% of the energy consumption of flash access). 

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{figures/energy.pdf}
%	\vspace{-5.5ex} 
%	\caption{Energy overhead of IceClave, normalized to ISC (left).}
%	\label{fig:energy}
%\end{figure}




\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/bws.pdf}
	\vspace{-5ex} 
	\caption{IceClave scales its performance, as we vary the internal SSD bandwidth by using different number of channels (normalized to Host).}
	\label{fig:bws}
		\vspace{-4ex}
\end{figure}



\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/bws-isc.pdf}
	\vspace{-6ex} 
	\caption{IceClave introduces minimal performance overhead (normalized to ISC), as we vary the internal SSD bandwidth by using different number of channels.}
	\label{fig:bws-isc}
		\vspace{-3ex}
\end{figure}

\subsection{Impact of SSD Bandwidth}
\label{subsec:bandwidth}
We now evaluate the performance sensitivity of IceClave, as we change different SSD parameters. 
We first vary the internal bandwidth of the SSD by changing the number of flash channels from 4 to 32. With this, 
the aggregated internal I/O bandwidth grows linearly, while the external bandwidth is 
capped by the PCIe bandwidth~\cite{summarizer, lightnvm}. We compare IceClave with the host-based approach (Host), 
and present the normalized speedup in Figure~\ref{fig:bws}. %As we can see, 
For each data query workload, 
the performance benefit of IceClave scales significantly, as we increase the number of channels. To be specific, 
IceClave speeds up the performance by 1.7--5.0$\times$ over Host, showing that IceClave has negligible 
negative impact on the performance of in-storage computing. As for in-storage workloads that involve 
more complicated computations such as TPC-B, TPC-C, and Wordcount, increasing the internal bandwidth brings 1.2--1.8$\times$ 
performance speedup, and for others such as the synthetic workloads and TPC-H, IceClave obtain more performance benefits (1.9-6.2$\times$).    
Note that IceClave achieves even more performance benefits than Host+SGX, because SGX introduces 
extra overhead (see Figure~\ref{fig:iscvsvanila} and $\S$\ref{subsec:perf}). 
And IceClave enables TEE for in-storage programs.
%\hl{For compute-intensive workloads SSJoin and decompress, we obtain trivial performance improvement as we 
%increase the SSD bandwidth, this is because these workloads are constrained by compute resources rather than I/O bandwidth.}

{As we vary the internal SSD bandwidth, we also compare IceClave with ISC. As shown in Figure}~\ref{fig:bws-isc}, 
{IceClave decreases the application performance by up to 28\% (8.6\% on average), compared to ISC. Its 
additional overhead is slightly 
increased as we increase the number of channels for complicated data queries like TPC-C. This is mainly due to the 
increased overhead of memory encryption and integrity verification. However, IceClave offers a TEE 
for offloaded programs, making us believe it is worth the effort. }



\subsection{Impact of Data Access Latency}
\label{subsec:latency}
To understand how the data access latency affects the performance of IceClave, 
{we vary the read latency of accessing a flash page from 10~$\mu$s, modeling an ultra-low 
latency NVMe SSD}~\cite{memblaze, optane_latency}, to 110~$\mu$s, modeling a commodity TLC-based SSD~\cite{microntlc}. 
We keep the write latency as 300~$\mu$s, this is because most in-storage workloads are read-intensive, 
which involve few write operations to the dataset stored 
in the SSD. We use 8 channels in the SSD. We present the experimental results in Figure~\ref{fig:lat}. 
{As shown in Figure}~\ref{fig:lat}, compared to the host-based computing approach that is bottlenecked by the 
external PCIe bandwidth, IceClave delivers performance benefit (1.8--3.2$\times$) for various 
SSD devices with different access latencies. For TPC-B, TPC-C, and TPC-H Q19 query workloads that 
require more computing resource for hash join operations, IceClave offers less performance 
benefit for the SSD with ultra-low latency, because the processors in the host machine provide more powerful computing resource. 
%\hl{For workloads SSJoin and decompress, their performance is not affected 
%by the data access latency significantly. This is expected as they are compute-bound.}


\subsection{Impact of Computing Capability}
\label{subsec:computing}
As we exploit embedded processors to run in-storage applications, 
it will be interesting to understand how the in-storage 
computing capability affects the efficiency of IceClave. 
%that more performance 
%benefit will come from more powerful embedded cores. 
We vary this parameter by using various models of embedded processor. We use our in-storage computing simulator to simulate 
the representative out-of-order (OoO) ARM processor A72, and the in-order processor A53 with different frequencies. 
We compare IceClave with the baseline Host that has an Intel i7-7700K processor running at 4.2GHz. 

We show the normalized speedup in Figure~\ref{fig:core_ipc}. The performance of IceClave drops 13.7--33.4\%
as we decrease the CPU frequency of ARM processors. And an OoO processor A72 performs slightly better than the in-order processor 
A53 with the same CPU frequency. This demonstrates that IceClave can work with different type of ARM processors and deliver 
reasonable performance benefits. 

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth, trim={0 0.3cm 0 0},clip]{figures/lat.pdf}
	\vspace{-3.8ex} 
	\caption{IceClave outperforms host-based computing for I/O-intensive workloads, as we vary the flash device latency.}
	\label{fig:lat}
		\vspace{-3ex}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/core_ipc.pdf}
	\vspace{-5.5ex} 
	\caption{Sensitivity analysis of IceClave, as we vary the in-storage computing capability.
	}
	\label{fig:core_ipc}
		\vspace{-3ex}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/dram.pdf}
	\vspace{-5.5ex} 
	\caption{Sensitivity analysis of IceClave, as we vary the DRAM size in the SSD controller.
	}
	\label{fig:dram-perf}
	\vspace{-3ex}
\end{figure}

\subsection{{Impact of DRAM Capacity in SSD}}
\label{subsec:dram}
{To evaluate the impact of the SSD DRAM capacity on the IceClave performance, we change the SSD DRAM size from 
4GB to 2GB while using the same configurations as described in Table}~\ref{tab:simconfig}. 
{We present the experimental results in Figure}~\ref{fig:dram-perf}. 
{As we decrease the SSD DRAM capacity, the performance of ISC drops by 12\%--44\%, as it has limited memory space to 
store its data set. The performance of IceClave follows the same trend. However, compared to ISC, IceClave still introduces 
minimal performance overhead.  
}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/twoclaves.pdf}
	\vspace{-6ex} 
	\caption{IceClave performance as we run two in-storage applications concurrently.
	}
	\label{fig:twoclaves}
	\vspace{-3ex}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/fourclaves.pdf}
	\vspace{-6ex} 
	\caption{IceClave performance as we run four in-storage applications concurrently.
	}
	\label{fig:fourclaves}
	\vspace{-3ex}
\end{figure}%ssss

\subsection{{Performance of Multi-tenant IceClave}}
\label{subsec:multitenant}
To further evaluate the efficiency of IceClave, 
we run multiple IceClave instances concurrently, and each instance hosts one of the 
in-storage workloads as described in Table~\ref{tab:workload}. 
We compare the application performance with the case of 
running each in-storage application independently without collocating with other instances. 
As shown in Figure~\ref{fig:twoclaves}, when we collocate the TPC-C instance with other 
workloads, the performance of in-storage applications is decreased by 6.1--15.7\%. 
As we increase the number of collocated instances (see Figure~\ref{fig:fourclaves}), 
their performance drops by 21.4\% on average. This is mainly caused by (1) the computational interference 
between the collocated IceClave instances, and (2) the increased cache misses (up to 8.7\%) 
of the cached mapping table in the protected memory region. 
%(which will cause context switches to the secure world for updating the mapping table entries). 
However, these in-storage programs still perform better 
than host-based approaches that are constrained by the external I/O bandwidth of SSDs. 
%As discussed in $\S$~\ref{subsec:overhead}, IceClave introduces minimal performance overhead to 
%in-storage programs, while ensuring their security isolation.  

==> implt.tex <==

\begin{table}[t]
    \centering
    \caption{Computational SSD simulator.}
    \vspace{-2ex}
    \footnotesize
    \label{tab:simconfig}
    \begin{tabular}{|l|l|}
        \hline
    	\textbf{SSD Processor}             & ARM Cortex-A72 1.6GHz{~\cite{www:smartssd,arm:storage}}                                  \\ \hline
        Decoder Width         & 3 ops                                                                                                 \\
        Disp/Retire Width & 5 ops \\                                                                          
        L1 I/D Cache          & 48KB/32KB                                                                                             \\
        L2 Cache              & 1MB                                                                                                 \\ \hline
        \textbf{SSD DRAM}  & DDR3 1600 MHz  \\ \hline              
        %	& \begin{tabular}[c]{@{}l@{}}4GB\\ 1 Channel\\ 2 Ranks/Channel\\ 8 Banks/Rank\end{tabular} \\ \hline
        	Capacity & 4GB \\
        	Organization & 1 Channel, 2 Ranks/Channel, 8 Banks/Rank \\
        	Timing & $t_{RCD}$-$t_{RAS}$-$t_{RP}$-$t_{CL}$-$t_{WR}$ = 11-28-11-11-12 \\
        %	Counter Cache:         & 128KB, 8-way, 64B lines, LRU                                                                          \\ 
        	Encryption Delay      & AES-128: 60ns                                                                                         \\ \hline
        \textbf{SSD}  & 1TB Flash-based SSD \\ \hline   
        	%Organization & 32 channels, 4 chips/channel, 8 planes/chip \\ 
        	%& 512 blocks/plane, 128 pages/block, 16KB/page \\ 
        	%Latency & 53$\mu$s for flash array access \\
        	%Bandwidth & 800 MB/s per channel \\ \hline
        	Organization & 8 channels, 4 chips/channel, 4 dies/chip \\
        	& 2 planes/die, 2048 blocks/plane \\
        	& 512 pages/block, 4KB page\\
        	& $t_{RD}$/$t_{WR}$=50/300$\mu$s\\
        	Bandwidth & 600 MB/sec per channel \\
    	\hline	
    \end{tabular}
    	\vspace{-2ex}
\end{table}


\section{Implementation Details}
\label{sec:implt}

\noindent
\textbf{Full System Simulator.}
We implement IceClave with a computational SSD simulator developed based on the
SimpleSSD~\cite{simplessd}, Gem5~\cite{gem5}, and USIMM~\cite{usimm} simulator.
This allows us to conduct the study with different SSD configurations, which cannot be 
easily conducted with a real SSD board. 
We use the SimpleSSD to simulate a modern SSD and its storage operations. 
We show the  
SSD configuration in Table~\ref{tab:simconfig}. 
%We assume a flash array access
%latency of 53$\mu$s, 16 channels, 4 flash chips per channel, 8 planes per chip, 512 blocks per plane,
%and 128 pages per block. Each flash page is 16KB in size and each flash channel has a bandwidth of 
%800MB/s~\cite{micronflashdiesize}.
To enable in-storage computing in the simulator, we utilize Gem5 to model the 
out-of-order ARM processor in the SSD controller. %(see the in-storage processor in Table~\ref{tab:simconfig}). 
%As discussed in $\S$~\ref{subsec:encryption}, 
We also implement the stream cipher in the integrated 
simulator to enable the data encryption/decryption as in-storage applications load data from flash chips. 
We use CACTI 6.5~\cite{cacti} to estimate its hardware cost, and find that the cipher engine introduces 
only 1.6\% area overhead to a modern SSD controller such as that of Intel DC P4500 SSD. 

As IceClave will enable the memory verification in SSD DRAM, we leverage USIMM to
simulate the DRAM in the SSD. We implement the Bonsai Merkle Tree (BMT) in the USIMM simulator, and 
use the hybrid-counter mode (see $\S$\ref{subsec:memory}) as the memory encryption scheme.
As discussed, the root of the integrity tree is stored in a 
secure on-chip register. The counter cache size is 128KB. %We use a 128KB cache for caching counters.
To enable memory encryption and integrity verification, we enforce that each memory access will  
trigger the verification and update of the MAC and integrity tree. 
As we develop a full system simulator with Gem5, we run real data-intensive workloads, such as 
transaction database to evaluate the efficiency of IceClave in the following section.  
%We use a 128KB dedicated metadata cache for caching counters.  
%We compare our proposed design: SC-128, following the split-counter scheme~\cite{encryption:isca06} against the a non-secure system and a SC-64 scheme, to illustrate the performance overhead imposed by our scheme.

\begin{figure}[t]
        \centering
        \includegraphics[width=0.85\linewidth]{figures/cipher_design-v2.pdf}
        \vspace{-2ex}
        \caption{Stream cipher engine design in IceClave.
        }
        \label{fig:cipher_design}
        	\vspace{-2ex}
\end{figure}


\noindent
\textbf{Real System Prototype.}
%In our simulator, we implement IceClave runtime using C progrmaming language. 
{To verify the core functions of IceClave, including TEE creation/deletion, FTL, and stream cipher engine, 
we also implement IceClave with an OpenSSD Cosmos+ FPGA board} that has a Dual ARM Cortex-A9 
processor~\cite{openssd-web}. We measure their overheads and show them in Table~\ref{tab:overhead}. 
%IceClave runtime will create a TEE when an application is offloaded to the SSD, and delete the 
%TEE when the offloaded in-storage application is completed or terminated. 
We demonstrate the architecture of the stream cipher engine in Figure~\ref{fig:cipher_design}.
Its key initialization block takes a symmetric key and an arbitrary initialization vector (IV) as the input
to initialize the cipher. IceClave keeps the key in a secure register, while the IV can be public.
Once initialized, the stream cipher generates 64 keystream bits per cycle.
The generated keystream is XORed bitwise with the data read from flash chips to produce the ciphered data.
%On the other side,
The decipher uses the same key and IV to decode the ciphered data.
%The IV needs to be unique during the entire process for security.
The IV is constructed with temporally unique random numbers and spatially unique address bits.
The orthogonal uniqueness enforces a strong guarantee that the same IV value will not be used twice 
during a certain period of time.
The stream cipher algorithm we used refers to the Trivium~\cite{Trivium}.
{To provide the uniqueness for different flash pages, we compose the IV by concatenating its physical page
address (PPA) and the output of a pseudo-random number generator (PRNG). }
%We implement the stream cipher engine in the SSD controller as follows.  %following the Trivium-64 scheme~\cite{Trivium, triadv1}. 
%It reads 288 state bits from the state register, produces 64 keystream bits, and generates 288 next-state bits.
%%Prior work~\cite{triadv1} reports a consumption of 3051 Gates Equivalent (GE) and 128.7$\mu$W. 
%%According to the energy modeling in~\cite{triadv1}, it takes only 10.3nJ to encrypt a 4KB flash page.
%Moreover, the stream cipher engine introduces minimal area overhead (1.6\% of the entire SSD controller) to a commodity SSD~\cite{flashctrl:fms17, onfi3:fms14}.
%


%To evaluate the performance of our design, we conduct cycle-accurate simulations with workloads from four essential database operations and benchmark suites: TPC-H. These workloads are described in Table x, along with their write ratio. We generate the memory traces for these workloads with PIN ~/cite{Pin}: the traces are generated for 1 billion memory accesses after fast-forwarding to the region of interest. These traces are then fed into cycle-accurate memory system simulator USIMM ~\cite{usimm}. USIMM parameters are listed in ~\tabref{tab:simconfig}, simulating a single-core Out-Of-Order ARM processor.




==> relatedwork.tex <==
\section{Related Work}
\label{sec:related}

\textbf{In-storage Computing.}
In-storage computing has been intensively developed recently. 
Researchers have been exploring it for applications such as
database query~\cite{summarizer,Do:2013:QPS:2463676.2465295,kang2013enabling,smartssd},
key-value store~\cite{willow}, map-reduce workloads~\cite{biscuit,kang2013enabling},
signal processing~\cite{ActiveFlash}, and scientific
data analysis~\cite{Tiwari:2013:AFT:2591272.2591286,Tiwari:2012:RDM:2387869.2387873}.
%They %treat the SSDs as compute device and leverage the embedded CPU processors
%utilize the embedded processors in the SSD controller
%to perform computing operations, such that it can move computation closer to the data for 
%avoiding large amount data transfer over PCIe. 
To enable in-storage computing in modern SSDs, 
these prior works have developed various frameworks~\cite{biscuit,willow,summarizer,insider:atc19}. 
However, most of them focus on the 
programmability and performance. %without paying much attention on the in-storage security. 
Although there is still space for improvement in these aspects, such as having SSD array and filesystem  
support for in-storage computing{~\cite{insider:atc19}}, we have to overcome the security challenge of in-storage computing for its widespread deployment, since it poses threats to user data and flash devices.
%As in-storage computing is being widely deployed in practice~\cite{samsungsmartssd, scaleflux}, 
%it poses threats to user data and storage devices. 
To the best of our knowledge, we are the first to propose building trusted execution environments for in-storage computing.  
%propose building trusted execution environments for in-storage computing. 
%To the best of our knowledge, we are the first 
%to propose building trusted execution environments for in-storage computing. 
%To the best of our knowledge, 
%we are the first to propose building trusted execution environments for in-storage computing. 

\textbf{Trusted Execution Environment.}
To defend applications from malicious systems software, trusted hardware  
devices have been developed. A typical example is Intel SGX~\cite{haven}, which can create 
trusted execution environments for applications. 
{Because of the enabled security isolation, SGX is extended or customized 
to support various computing platforms}~\cite{graviton:osdi2018, scone:osdi2016, obliviate, pesos:eurosys2018, sanctum:usenixsec2016} {and 
applications}~\cite{vc3:oakland2015, enclavedb, shieldstore:eurosys2019, speicher:fast2019}. 
The hardware devices with TPM~\cite{tpm} serve the similar purpose by utilizing 
the attestation available in commodity processors from AMD and 
Intel~\cite{flicker,logicalattestation,trustvisor}. 
For ARM processors that are commonly used in 
mobile devices and storage controllers, they offer TrustZone that enables users 
to create secure world isolated from the OS~\cite{vtz, trustzone:asplos14}. Unfortunately, none of these hardware devices can be directly applied 
to in-storage computing. %and defend against physical attacks. 
%{For instance, %Guardat}~\cite{guardat:eurosys2015} {and Pesos}~\cite{pesos:eurosys2018} {allow 
%users to specify security policies in storage devices to protect data confidentiality and integrity, 
The most recent work 
ShieldStore~\cite{shieldstore:eurosys2019} {and Speicher}~\cite{speicher:fast2019} {applied SGX to key-value stores, however, none of them can protect 
the execution of in-storage programs.} 
We develop specific trusted execution environments for in-storage applications. 
%for security isolation with minimal hardware cost. 

\textbf{Storage Encryption and Security.} 
As we move computation closer to data in the storage devices, it would inevitably increase 
the trusted computing base, which poses security threats to user data. To protect sensitive user 
data while enabling near-data computing, a common approach is data encryption~\cite{denfs}. 
However, data leakage 
or loss would still happen at runtime, due to the lack of TEE support in 
modern SSD controllers. And adversaries can also initiate physical attacks to steal/destroy user data. 
An alternative approach is to enable computation on encrypted data~\cite{opaque:nsdi17, ocq:eurosys2020}. 
However, such an approach requires 
intensive computing resource, which cannot be satisfied by modern SSD controllers due to the 
limited resource budget~\cite{deepstore:micro2019, neardata, biscuit, timessd:eurosys2019}. 
Our work IceClave presents a lightweight approach that can enforce security isolation for in-storage 
applications as well as defend against physical attacks. 


==> runtime.tex <==
\subsection{IceClave Runtime}
\label{subsec:runtime}
In this section, we discuss how IceClave runtime facilitates the execution of in-storage TEEs. 
%IceClave runtime is developed based on the ARM TrustZone with the security techniques we discussed in previous sections.  
It provides the essential functions for managing in-storage TEEs, such as TEE setup, TEE lifecycle 
and metadata management, and the interaction with the secure world. 
%It is the software measure that extends our proposed security features for in-storage-computing based on ARM TrustZone. 
IceClave runtime also interacts with IceClave library deployed in the host machine. Note that 
IceClave library only exposes basic offloading interfaces (e.g., RPC) to end users. 
This not only reduces the trusted computing base but also simplifies the development of in-storage programs. 
We list the APIs of IceClave in Table~\ref{tab:api}. 

IceClave allows a user to interact with the SSD using two APIs: \texttt{OffloadCode} and \texttt{GetResult}. 
Once the program is offloaded to the SSD, IceClave runtime will execute \texttt{CreateTEE()} to create 
a new TEE. %Upon successful return, the TEE is initialized and gets an TEE ID. 
At the same time, 
it will call \texttt{SetIDBits()} to set the ID bits (access permission, see $\S$\ref{subsec:mapping}) 
of the corresponding address mapping table entries in FTL with the list of logical page addresses specified 
by the in-storage program. According to our study on the popular in-storage programs, their code size 
is 28--528KB. However, for an offloaded program whose size is larger than the available space of SSD DRAM, 
the TEE creation will fail.
During the execution of an in-storage program, \texttt{ThrowOutTEE()} will be called to handle program 
exceptions. IceClave runtime will abort the TEE for these cases that include (1) access control is violated, 
(2) TEE memory or metadata is corrupted, and (3) in-storage program throws an exception.
Once the in-storage program is finished, IceClave runtime will call the \texttt{TerminateTEE()} to terminate 
the TEE. %reclaim its allocated memory, and its TEE ID. %Once this is performed, the TEE can no longer be accessed via any means.
%We will describe the detailed workflow in the following section. 

With the assistance of TrustZone, IceClave supports dynamic memory allocation within each TEE. To avoid 
memory fragmentation, IceClave will preallocate a large contiguous memory region (16MB by default). Upon 
TEE deletion, IceClave runtime will release the preallocated memory region.


